Functional Encryption with Secure Key Leasing

Secure software leasing is a quantum cryptographic primitive that enables us to lease software to a user by encoding it into a quantum state. Secure software leasing has a mechanism that verifies whether a returned software is valid or not. The security notion guarantees that once a user returns a software in a valid form, the user no longer uses the software. In this work, we introduce the notion of secret-key functional encryption (SKFE) with secure key leasing, where a decryption key can be securely leased in the sense of secure software leasing. We also instantiate it with standard cryptographic assumptions. More specifically, our contribution is as follows. - We define the syntax and security definitions for SKFE with secure key leasing. - We achieve a transformation from standard SKFE into SKFE with secure key leasing without using additional assumptions. Especially, we obtain bounded collusion-resistant SKFE for P/poly with secure key leasing based on post-quantum one-way functions since we can instantiate bounded collusion-resistant SKFE for P/poly with the assumption. Some previous secure software leasing schemes capture only pirate software that runs on an honest evaluation algorithm (on a legitimate platform). However, our secure key leasing notion captures arbitrary attack strategies and does not have such a limitation. We also introduce the notion of single-decryptor FE (SDFE), where each functional decryption key is copy-protected. Since copy-protection is a stronger primitive than secure software leasing, this notion can be seen as a stronger cryptographic primitive than FE with secure key leasing. More specifically: - We define the syntax and security definitions for SDFE. - We achieve collusion-resistant single-decryptor PKFE for P/poly from post-quantum indistinguishability obfuscation and quantum hardness of the learning with errors problem.

==> flawed_single_dec_FE.tex <==
% !TEX root = ../main.tex


\section{Single-Decryptor Functional Encryption}\label{sec:single_dec_FE}
This section introduces single-decryptor FE (SDFE), whose functional decryption keys are copy-protected.

\subsection{Preliminaries for SDFE}

\input{section/quantum_information}

\paragraph{Cryptographic tools.}
\fuyuki{Do we need the def of LWE?}\ryo{We use it for SDFE though we do not directly use it. In the submission, most preliminaries will be move to appendix, so leaving it is ok, but you can delete it.}
\begin{definition}[Learning with Errors]\label{def:LWE}
Let $n,m,q \in \N$ be integer functions of the security parameter $\secp$. Let $\chi = \chi(\secp)$ be an error distribution over $\Z$.
The LWE problem $\LWE_{n,m,q,\chi}$ is to distinguish the following two distributions.
\ifnum\llncs=0
\[
D_0 \seteq \setbracket{(\mm{A},\mv{s}^{\intercal}\mm{A}+\mv{e}) \mid \mm{A} \chosen \Zq^{n\times m}, \mv{s}\chosen \Zq^{n}, \mv{e}\chosen \chi^m}  \text{ and } D_1 \seteq \setbracket{(\mm{A},\mv{u}) \mid \mm{A} \chosen \Zq^{n\times m}, \mv{u}\chosen \Zq^m}.
\]
\else
\begin{align}
&D_0 \seteq \setbracket{(\mm{A},\mv{s}^{\intercal}\mm{A}+\mv{e}) \mid \mm{A} \chosen \Zq^{n\times m}, \mv{s}\chosen \Zq^{n}, \mv{e}\chosen \chi^m}  \text{ and }\\
&D_1 \seteq \setbracket{(\mm{A},\mv{u}) \mid \mm{A} \chosen \Zq^{n\times m}, \mv{u}\chosen \Zq^m}.
\end{align}
\fi

When we say we assume the hardness of the LWE problem or the QLWE assumption holds, we assume that for any QPT adversary $\qalgo{A}$, it holds that
\[
\abs{ \Pr[\qA (D_0)\out  1 ] - \Pr[\qA (D_1)\out 1]} \le \negl(\secp).
\]
\end{definition}

\begin{definition}[Puncturable PRF]\label{def:pprf}
A puncturable PRF (PPRF) is a tuple of algorithms $\PuncPRF = (\prfgen, \prf,\Puncture)$ where $\{\prf_{K}: \bin^{\ell_1} \ra \zo{\ell_2} \mid K \in \zo{\secp}\}$ is a PRF family and satisfies the following two conditions. Note that $\ell_1$ and $\ell_2$ are polynomials of $\secp$.
   \begin{description}
       \item[Punctured correctness:] For any polynomial-size set $S \subseteq \zo{\ell_1}$ and any $x\in \zo{\ell_1} \setminus S$, it holds that
       \begin{align}
       \Pr[\prf_{K}(x) = \prf_{K_{\notin S}}(x)  \mid K \gets \prfgen(1^{\secp}),
       K_{\notin S} \gets \Puncture(K,S)]=1.
       \end{align}
       \item[Pseudorandom at punctured point:] For any polynomial-size set $S \subseteq\zo{\ell_1}$
       and any QPT distinguisher $\qA$, it holds that
       \begin{align}
       \vert
       \Pr[\qA(\prf_{K_{\notin S}},\{\prf_{K}(x_i)\}_{x_i\in S}) \out 1] -
       \Pr[\qA(\prf_{K_{\notin S}}, (\cU_{\ell_2})^{\abs{S}}) \out 1]
       \vert \leq \negl(\secp),
       \end{align}
       where $K\gets \prfgen(1^{\secp})$,
       $K_{\notin S} \gets \Puncture(K,S)$ and $\cU_{\ell_2}$ denotes the uniform distribution over $\zo{\ell_2}$.
   \end{description}
   If $S = \setbk{x^\ast}$ (i.e., puncturing a single point), we simply write $\prf_{\ne x^\ast}(\cdot)$ instead of $\prf_{K_{\notin S}}(\cdot)$ and consider $\prf_{\ne x^\ast}$ as a keyed function.
\end{definition}

It is easy to see that the Goldwasser-Goldreich-Micali tree-based construction of PRFs (GGM PRF)~\cite{JACM:GolGolMic86} from \rmOWF yield puncturable PRFs where the size of the punctured key grows polynomially with the size of the set $S$ being punctured~\cite{AC:BonWat13,PKC:BoyGolIva14,CCS:KPTZ13}. Thus, we have:
\begin{theorem}[\cite{JACM:GolGolMic86,AC:BonWat13,PKC:BoyGolIva14,CCS:KPTZ13}]\label{thm:pprf-owf} If OWFs exist, then for any polynomials $\ell_1(\secp)$ and $\ell_2(\secp)$, there exists a PPRF that maps $\ell_1$-bits to $\ell_2$-bits.
\end{theorem}


\begin{definition}[Public-Key Functional Encryption]\label{def:PKFE}
A PKFE scheme $\PKFE$ is a tuple of four PPT algorithms $(\Setup, \KG, \Enc, \Dec)$. 
Below, let $\cX$, $\cY$, and $\cF$ be the plaintext, output, and function spaces of $\PKFE$, respectively.
\begin{description}
\item[$\Setup(1^\secp)\ra(\pk,\msk)$:] The setup algorithm takes a security parameter $1^\secp$ and outputs a public key $\pk$ and master secret key $\msk$.
\item[$\KG(\msk,f)\ra\sk_f$:] The key generation algorithm $\KG$ takes a master secret key $\msk$ and a function $f \in \cF$, and outputs a functional decryption key $\sk_f$.

\item[$\Enc(\pk,x)\ra\ct$:] The encryption algorithm takes a public key $\pk$ and a message $x \in \cX$, and outputs a ciphertext $\ct$.

\item[$\Dec(\sk_f,\ct)\ra y$:] The decryption algorithm takes a functional decryption key $\sk_f$ and a ciphertext $\ct$, and outputs $y \in \{ \bot \} \cup \cY$.

\item[Correctness:] We require 
we have that
\[
\Pr\left[
\Dec(\sk_f, \ct) = f(x)
 \ \middle |
\begin{array}{rl}
 &(\pk,\msk) \la \Setup(1^\secp),\\
 & \sk_f \gets \KG(\msk,f), \\
 &\ct \gets \Enc(\msk,x)
\end{array}
\right]=1 -\negl(\secp).
\]
\end{description}
\end{definition}
Note that $\Setup$ does not take collusion bound $1^q$ unlike SKFE in~\cref{def:SKFE} since we consider only single-key and collusion-resistant PKFE in this work.


\begin{definition}[Adaptive Indistinguishability-Security for PKFE]\label{def:ad_ind_PKFE}
We say that $\PKFE$ is an \emph{adaptively indistinguishability-secure} SDFE scheme for $\Xs,\Ys$, and $\Fs$, if it satisfies the following requirement, formalized from the experiment $\expb{\qA}{ada}{ind}(1^\secp,\coin)$ between an adversary $\qA$ and a challenger:
        \begin{enumerate}
            \item The challenger runs $(\pk,\msk)\gets\Setup(1^\secp)$ and sends $\pk$ to $\qA$.
            \item $\qA$ sends arbitrary key queries. That is, $\qA$ sends function $f_{i}\in\Fs$ to the challenger and the challenger responds with $\sk_{f_i}\gets \KG(\msk,f_i)$ for the $i$-th query $f_{i}$.
            \item At some point, $\qA$ sends $(x_0,x_1)$ to the challenger. If $f_i(x_0)=f_i(x_1)$ for all $i$, the challenger generates a ciphertext $\ct^*\gets\Enc(\pk,x_\coin)$. The challenger sends $\ct^*$ to $\qA$.
            \item Again, $\qA$ can sends function queries $f_i$ such that $f_i(x_0)=f_i(x_1)$.
            \item $\qA$ outputs a guess $\coin^\prime$ for $\coin$.
            \item The experiment outputs $\coin^\prime$.
% if $f_i(m_0^*) = f_i(m_1^*)$ for all $i\in [q_k]$ and $\bot$ otherwise.
        \end{enumerate}
        We say that $\PKFE$ is adaptively indistinguishability-secure if, for any QPT $\qA$, it holds that
\begin{align}
%\adva{\A}{sel} \set \Pr\left[\expt{A}{sel} (1^\secp,0)=1\right] - \Pr\left[\expt{\A}{sel}(1^\secp,1)=1\right] \leq \mu(\secp).
\advb{\PKFE,\qA}{ada}{ind}(\secp) \seteq \abs{\Pr[\expb{\PKFE,\qA}{ada}{ind} (1^\secp,0) \out 1] - \Pr[\expb{\PKFE,\qA}{ada}{ind} (1^\secp,0) \out 1] }\leq \negl(\secp).
\end{align}
If $\qA$ can send only one key query during the experiment, we say $\PKFE$ is adaptively single-key indistinguishability-secure.
\end{definition}


\begin{theorem}[\cite{C:GorVaiWee12}]\label{thm:pkfe_from_pke}
If there exists PKE, there exists adaptively single-key indistinguishability-secure PKFE for $\Ppoly$.
\end{theorem}

% \begin{theorem}[\cite{EC:KNYY21}]\label{thm:perfect_correct_pke_lwe}
% If the QLWE assumption holds, there exists PKE that satisfies perfect correctness.
% \end{theorem}


\begin{definition}[Indistinguishability Obfuscator~\cite{JACM:BGIRSVY12}]\label{def:io}
A PPT algorithm $\iO$ is a secure \rmIO for a classical circuit class $\{\cC_\secp\}_{\secp \in \bbN}$ if it satisfies the following two conditions.

\begin{description}
\item[Functionality:] For any security parameter $\secp \in \bbN$, circuit $C \in \cC_\secp$, and input $x$, we have that
\begin{align}
\Pr[C^\prime(x)=C(x) \mid C^\prime \lrun \iO(C)] = 1\enspace.
\end{align}


\item[Indistinguishability:] For any PPT $\Sampler$ and QPT distinguisher $\qD$, the following holds:

If $\Pr[\forall x\ C_0(x)=C_1(x) \land \abs{C_0}=\abs{C_1} \mid (C_0,C_1,\aux)\gets \Sampler(1^\secp)]> 1 - \negl(\secp)$, then we have
 \begin{align}
\adva{\iO,\qD}{io}(\secp) &\seteq \left|
 \Pr\left[\qD(\iO(C_0),\aux) = 1 \mid (C_0,C_1,\aux)\gets \Sampler(1^\secp) \right] \right.\\
&~~~~~~~ \left. - \Pr\left[\qD(\iO(C_1),\aux)= 1\mid (C_0,C_1,\aux)\gets \Sampler(1^\secp)  \right] \right|
  \leq \negl(\secp).
 \end{align}
\end{description}
\end{definition}


There are a few candidates of secure IO for polynomial-size classical circuits against quantum adversaries~\cite{TCC:BGMZ18,TCC:CHVW19,EC:AgrPel20,myTCC:DQVWW21}.




\subsection{Single-Decryptor Encryption}\label{sec:single_dec_PKE}

We review the notion of single-decryptor encryption (SDE)~\cite{EPRINT:GeoZha20,C:CLLZ21} since it is a crucial building block of our SDFE schemes.
We also extend the existing definitions for SDE.
Some definitions are taken from the paper by Coladangelo et al.~\cite{C:CLLZ21}.
\begin{definition}[Single-Decryptor Encryption~\cite{C:CLLZ21}]\label{def:single_dec_PKE}
A single-decryptor encryption scheme $\SDE$ is a tuple of four algorithms $(\Setup, \QKeyGen, \Enc, \qDec)$. 
Below, let $\calM$ be the message space of $\SDE$.
\begin{description}
\item[$\Setup(1^\secp)\ra(\pk,\sk)$:] The setup algorithm takes a security parameter $1^\secp$, and outputs a public key $\pk$ and a secret key $\sk$.
\item[$\QKeyGen(\sk)\ra\qsk$:] The key generation algorithm $\QKeyGen$ takes a secret key $\sk$, and outputs a quantum decryption key $\qsk$.
\item[$\Enc(\pk,m)\ra\ct$:] The encryption algorithm takes a public key $\pk$ and a message $m \in \calM$, and outputs a ciphertext $\ct$.
\item[$\qDec(\qsk,\ct)\ra\tilde{m}$:] The decryption algorithm takes a quantum decryption key $\qsk$ and a ciphertext $\ct$, and outputs a message $\tilde{m} \in \{ \bot \} \cup \calM$.

\item[Correctness:] We require $\qDec(\qsk, \ct) \allowbreak = m$ for every $m \in \calM$, $(\sk,\pk) \la \Setup(1^\secp)$, $\qsk\gets\QKeyGen(\sk)$, and $\ct\gets\Enc(\pk,m)$.
\end{description}
\end{definition}
Note that $\Setup$ and $\Enc$ are classical algorithms.
Although they could be quantum algorithms, we select the definition above since the construction by Coladangelo et al.~\cite{C:CLLZ21} satisfies it.
This property is crucial in our schemes.

\begin{definition}[CPA Security]\label{def:single_dec_PKE_CPA}
An SDE scheme satisfies CPA security if for any (stateful) QPT $\qA$, it holds that
\[
2\abs{\Pr\left[
\qA(\ct_b)=b
 \ \middle |
\begin{array}{rl}
 &(\pk,\sk)\lrun \Setup(1^\secp),\\
 &(m_0,m_1) \lrun \qA(\pk), b \chosen \zo{}, \\
 &\ct_b \lrun \Enc(\pk,m_b)
 \end{array}
\right] -\frac{1}{2}} \le  \negl(\secp).
\]
\end{definition}

\begin{definition}[Quantum Decryptor~\cite{C:CLLZ21}]\label{def:qunatum_decryptor}
Let $\qstate{p}$ and $\mat{U}$ be a quantum state and a general quantum circuit acting on $n+m$ qubits, where $m$ is the number of qubits of $\qstate{p}$ and $n$ is the length of ciphertexts. A quantum decryptor for ciphertexts is a pair $(\qstate{p},\mat{U})$.

When we say that we run the quantum decryptor $(\qstate{p},\mat{U})$ on ciphertext $\ct$, we execute the circuit $\mat{U}$ on inputs $\ket{\ct}$ and $\qstate{p}$.
\end{definition}


Coladangelo et al.~\cite{C:CLLZ21} introduced a few security notions for SDE.
We introduce the stronger security notion among them, $\gamma$-anti-piracy security.

\begin{definition}[Testing a Quantum Decryptor~\cite{C:CLLZ21}]\label{def:test_quantum_decryptor}
Let $\gamma \in [0,1]$. Let $\pk$ and $(m_0,m_1)$ be a public key and a pair of messages, respectively.
A test for a $\gamma$-good quantum decryptor with respect to $\pk$ and $(m_0,m_1)$ is the following procedure.
\begin{itemize}
\item The procedure takes as input a quantum decryptor $\pirateD =(\qstateq,\mat{U})$.
\item Let $\cP = (\mat{P}, \mat{I} - \mat{P})$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
\begin{itemize}
\item Sample a uniformly random $\coin\chosen \bit$ and compute $\ct \gets \Enc(\pk,m_\coin)$.
\item Run $m^\prime \gets \pirateD(\ct)$. If $m^\prime = m_\coin$, output $1$, otherwise output $0$.
\end{itemize}
Let $\TI_{1/2+\gamma}(\cP)$ be the threshold implementation of $\cP$ with threshold $\frac{1}{2}+\gamma$.
Apply $\TI_{1/2+\gamma}(\cP)$ to $\qstateq$. If the outcome is $1$, we say that the test passed, otherwise the test failed.
\end{itemize}
\end{definition}

% \begin{corollary}[$\gamma$-good Decryptor~\cite{C:CLLZ21}]
% Let
% \begin{itemize}
% \item $\gamma \in [0,1]$
% \item $(\qstateq,\mat{U})$ be a quantum decryptor
% \item $\TI_{1/2 + \gamma}(\cP)$ be the test for a $\gamma$-good decryptor defined in~\cref{def:test_quantum_decryptor}.
% \end{itemize}
% We refer to states which are in the span of all eigenvectors of $\mat{P}$ with eigenvalues at least $1/2+\gamma$ as a $\gamma$-good decryptor with respect to $(m_0,m_1)$. Note that $\cP=(\mat{P},\mat{I}-\mat{P})$.
% Then, the post-measurement state conditioned on output $1$ is a mixture of $\gamma$-good decryptor with respect to $\pk$ and $(m_0,m_1)$.
% \end{corollary}

\begin{definition}[Strong Anti-Piracy Security~\cite{C:CLLZ21}]\label{def:strong_anti-piracy_PKE}
Let $\gamma \in [0,1]$.
We consider the strong $\gamma$-anti-piracy game $\expc{\SDE,\qA}{strong}{anti}{piracy}(\secp,\gamma(\secp))$ between the challenger and an adversary $\qA$ below.
\begin{enumerate}
\item The challenger generates $(\pk,\sk)\gets \Setup(1^\secp)$.
\item The challenger generates $\qsk \gets \QKeyGen(\sk)$ and sends $(\pk,\qsk)$ to $\qA$.
\item $\qA$ outputs $(m_0,m_1)$ and two (possibly entangled) quantum decryptors $\pirateD_1 = (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2 = (\qstateq[\qreg{R}_2],\mat{U}_2)$, where $m_0 \ne m_1$, $\abs{m_0}=\abs{m_1}$, $\qstateq$ is a quantum state over registers $\qreg{R}_1$ and $\qreg{R}_2$, and $\mat{U}_1$ and $\mat{U}_2$ are general quantum circuits.
\item The challenger runs the test for a $\gamma$-good decryptor with respect to $(m_0,m_1)$ on $\pirateD_1$ and $\pirateD_2$.
The challenger outputs $1$ if both tests pass; otherwise outputs $0$.
\end{enumerate}

We say that $\SDE$ is strong $\gamma$-anti-piracy secure if for any QPT adversary $\qA$, it satisfies that
\[
\Pr[\expc{\SDE,\qA}{strong}{anti}{piracy}(\secp,\gamma(\secp))=1]  \le  \negl(\sep).
\]
\end{definition}

\begin{theorem}[\cite{C:CLLZ21,ARXIV:CulVid21}]
Assuming the existence of sub-exponentially secure IO for $\Ppoly$ and OWFs, the hardness of QLWE, there exists an SDE scheme that satisfies strong $\gamma$-anti-piracy security for any inverse polynomial $\gamma$.
\end{theorem}

\paragraph{Extension of SDE.}
We define a more liberal security notion for $\gamma$-anti-piracy security of SDE to use an SDE scheme as a building block of some cryptographic primitive.
% We first define a few notions.
% \begin{definition}[Injective Randomized Function]\label{def:injective_rand_function}
% A randomized function $g: \Dom \times \cR \ra \Rng$ is injective if for all distinct $x_0,x_1\in \Dom$, there is no $r_0,r_1 \in \cR$ such that
% \[
% g(x_0;r_0) = g(x_1;r_1).
% \]
% Here, $\Dom$, $\Rng$, and $\cR$ are the domain, range, and randomness space of $g$, respectively.
% \end{definition}


We define a slightly stronger version of quantum decryptor than that in~\cref{def:qunatum_decryptor}.
\begin{definition}[Testing a Quantum Distinguisher for Randomized Message]\label{def:test_quantum_decryptor_rand_msg}
Let $\gamma \in [0,1]$. Let $\pk$ and $(m_0,m_1)$ be a public key and a pair of messages, respectively. Let $\cG=\setbk{\cG_\secp}_{\secp \in \N}$ be a function family.
A test for a $\gamma$-good quantum distinguisher with respect to $\pk$ and $(m_0,m_1,g \in \cG_\secp)$ is the following procedure.
\begin{itemize}
\item The procedure takes as input a quantum decryptor $\pirateD =(\qstateq,\mat{U})$.
\item Let $\cP = (\mat{P}, \mat{I} - \mat{P})$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
\begin{itemize}
\item Sample a uniformly random $\coin\chosen \bit$ and $r \chosen \cR$, and compute $\ct \gets \Enc(\pk,g(m_\coin;r))$.
\item Run $\coin^\prime \gets \pirateD(\ct)$. If $\coin^\prime = \coin$, output $1$, otherwise output $0$.
\end{itemize}
Let $\TI_{1/2+\gamma}(\cP)$ be the threshold implementation of $\cP$ with threshold $\frac{1}{2}+\gamma$.
Apply $\TI_{1/2+\gamma}(\cP)$ to $\qstateq$. If the outcome is $1$, we say that the test passed, otherwise the test failed.
\end{itemize}
\end{definition}
The definition above is different from~\cref{def:test_quantum_decryptor}. First, we apply a randomized function to $m_\coin$ and encrypt $g(m_\coin;r)$. Second, $\pirateD$ distinguish whether $\ct$ is a ciphertext of $g(m_0;r)$ or $g(m_1;r)$ rather than computing $g(m_\coin;r)$ (or $m_\coin$).
These differences are crucial when using SDE as a building block of some cryptographic primitive.

% \begin{corollary}[$\gamma$-good Distinguisher for randomized function $g$]\label{cor:gamma_good_dec_g}
% \fuyuki{We do not need this? We discussed that \cite{C:CLLZ21} needed this corollary for extraction.}
% Let
% \begin{itemize}
% \item $\gamma \in [0,1]$
% \item $(\qstateq,\mat{U})$ be a quantum decryptor
% \item $\TI_{1/2 + \gamma}(\cP)$ be the test for a $\gamma$-good distinguisher with respect to $\pk$ and $(m_0,m_1,g)$ defined in~\cref{def:test_quantum_decryptor_rand_msg}.
% \end{itemize}
% We refer to states which are in the span of all eigenvectors of $\mat{P}$ with eigenvalues at least $1/2+\gamma$ as a $\gamma$-good distinguisher with respect to $\pk$ and $(m_0,m_1,g)$. Note that $\cP=(\mat{P},\mat{I}-\mat{P})$.
% Then, the post-measurement state conditioned on output $1$ is a mixture of $\gamma$-good distinguisher with respect to $\pk$ and $(m_0,m_1,g)$.
% \end{corollary}

We finished preparation for defining a new security notion for SDE.
In the security game defined below, the adversary can send a randomized function applied to challenge messages by the challenger.
\begin{definition}[Strong Anti-Piracy Security for Randomized Message]\label{def:strong_anti-piracy_rand_msg_PKE}
Let $\gamma \in [0,1]$.
We consider the strong $\gamma$-anti-piracy with randomized function family $\cG=\setbk{\cG_\secp}_{\secp \in \N}$ game $\expd{\SDE,\qA,\cG}{strong}{anti}{piracy}{rand}(\secp,\gamma(\secp))$ between the challenger and an adversary $\qA$ below.
\begin{enumerate}
\item The challenger generates $(\pk,\sk)\gets \Setup(1^\secp)$.
\item The challenger generates $\qsk \gets \QKeyGen(\sk)$ and sends $(\pk,\qsk)$ to $\qA$.
\item $\qA$ outputs $(m_0,m_1)$, $g\in \cG_\secp$, and two (possibly entangled) quantum decryptors $\pirateD_1 = (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2 = (\qstateq[\qreg{R}_2],\mat{U}_2)$, where $\abs{m_0}=\abs{m_1}$, $\qstateq$ is a quantum state over registers $\qreg{R}_1$ and $\qreg{R}_2$, and $\mat{U}_1$ and $\mat{U}_2$ are general quantum circuits.
\item The challenger runs the test for a $\gamma$-good distinguisher with respect to $\pk$ and $(m_0,m_1,g)$ on $\pirateD_1$ and $\pirateD_2$.
The challenger outputs $1$ if both tests pass; otherwise outputs $0$.
\end{enumerate}

We say that $\SDE$ is strong $\gamma$-anti-piracy secure with randomized function family $\cG$ if for any QPT adversary $\qA$, it satisfies that
\[
\Pr[\expd{\SDE,\qA,\cG}{strong}{anti}{piracy}{rand}(\secp,\gamma(\secp))=1]  \le  \negl(\sep).
\]
\end{definition}
Note that we remove the restriction $m_0\ne m_1$, which is in~\cref{def:strong_anti-piracy_PKE}, since the adversary has no advantage even if it sets $m_0 =m_1$.

We do not know how to prove that an SDE scheme that satisfies strong $\gamma$-anti-piracy secure also satisfies strong $\gamma$-anti-piracy secure with randomized function in a black-box way.
This is because the adversary $\qA$ does not receive a challenge ciphertext, but quantum decryptor $\pirateD_1$ and $\pirateD_2$ receives it. That is, a reduction that plays the role of $\qA$ does not receive the challenge ciphertext.
\footnote{In the standard PKE setting, it is easy to see that the standard CPA security implies the liberal CPA security variant, where the adversary select not only $(m_0,m_1)$ but also $g\in \cG_\secp$.}

However, it is easy to see that the SDE scheme by Coladangelo et al.~\cite{C:CLLZ21} satisfies strong $\gamma$-anti-piracy secure with randomized function family $\cG$.
Intuitively, selecting $g$ does not give more power to adversaries since they can select \emph{any} $(m_0,m_1)$ in the original strong anti-piracy security.
We can easily obtain the following theorem.
\begin{theorem}[\cite{C:CLLZ21,ARXIV:CulVid21}]\label{thm:SDE_rand_from_IO_LWE}
Assuming the existence of sub-exponentially secure IO for $\Ppoly$ and OWFs, the hardness of QLWE, and $\cG$ is a randomized function family, there exists an SDE scheme that satisfies strong $\gamma$-anti-piracy security with randomize function family $\cG$ for any inverse polynomial $\gamma$.
\end{theorem}

The proof of~\cref{thm:SDE_rand_from_IO_LWE} is almost the same as that of the strong anti-piracy security of the SDE by Coladangelo et al.~\cite[Theorem 6.13 in the eprint ver.]{C:CLLZ21}.
We explain only the differences to avoid replication.
\paragraph{On randomized message.}
To obtain this theorem, we simply replace $m_b$ with $g(m_b;r_b)$ in the proof by Coladangelo et al.~\cite[Section 6.4 in the ePrint ver.]{C:CLLZ21}, where $r_b$ is randomness chosen by the challenger.
The intuition is as follows.
Even if the challenger applies the adversarially chosen randomized function $g$ to $m_0$ or $m_1$, it does not give more power to the adversary for breaking strong $\gamma$-anti-piracy security. This is because the adversary can send \emph{any} two messages $(m_0,m_1)$ as a challenge message pair in the original strong $\gamma$-anti-piracy security game. The proof by Coladangelo et al.~\cite{C:CLLZ21} does not use any specific property of challenge messages.
The one issue is whether $g(m_0;r_0)\ne g(m_1;r_1)$ holds for any $r_0,r_1 \in \cR$ since the original strong $\gamma$-anti-piracy game requires that challenge messages must be different.
However, this restriction is just a convention. If the adversary sets $m_0=m_1$, it just loses how to distinguish ciphertexts.
That is, even if $g(m_0;r_0)= g(m_1;r_1)$ happens, it does not give more power to the adversary, and is not a problem.

\paragraph{On distinguish-based definition.}
We require a pirate to be a distinguisher rather than a decryptor (computing entire $m_\coin$).
In general, security against distinguisher-based pirates is not implied by security against decryptor-based pirates since adversaries do not need to compute the entire $m_\coin$ in the distinguisher-based definition (the requirement on adversaries is milder).

In the original proof by Coladangelo et al.~\cite{C:CLLZ21}, they show that if pirate decryptors compute $m_\coin$, the reduction can distinguish whether a ciphertext is a real compute-and-compare obfuscation or a simulated compute-and-compare obfuscation.\footnote{The SDE scheme by Coladangelo et al.~\cite{C:CLLZ21} is constructed from IO and compute-and-compare obfuscation~\cite{FOCS:WicZir17,FOCS:GoyKopWat17}.} This breaks the unpredictability of the supported distribution in compute-and-compare obfuscation. Thus, pirate decryptors cannot compute $m_\coin$.
Here, even if pirate decryptors only distinguish $m_0$ from $m_1$ (that is, the output of $\pirateD$ is only one-bit information) instead of computing entire $m_\coin$, the reduction can distinguish real or simulation for compute-and-compare obfuscation. This is because the security of compute-and-compare obfuscation is the decision-type. The reduction in the original proof use only information about $\coin$ and \emph{does not use $m_\coin$}. Thus, we can prove strong $\gamma$-anti-piracy security with any randomized function family $\cG$ defined in~\cref{def:strong_anti-piracy_rand_msg_PKE}.

\paragraph{Other security notions for SDE.}
Coladangelo et al. introduced a few variants of anti-piracy security~\cite{C:CLLZ21}.
One is the CPA-style anti-piracy security, and the other is the anti-piracy security with random challenge plaintexts.
Both are weaker than the strong anti-piracy security in the SDE setting.
See~\cref{def:anti-piracy_CPA_PKE} for the CPA-style definition. We omit the anti-piracy security with random challenge plaintexts since we do not use it in this work.


\subsection{Definitions for Single-Decryptor Functional Encryption}\label{sec:def_single_dec_FE}
We define the notion of single-decryptor functional encryption (SDFE).

\begin{definition}[Single-Decryptor Functional Encryption]\label{def:single_dec_FE}
A single-decryptor functional encryption scheme $\SDFE$ is a tuple of five algorithms $(\Setup,\allowbreak\KG, \QKeyGen, \Enc, \qDec)$. 
Below, let $\cX$, $\cY$, and $\cF$ be the plaintext, output, and function spaces of $\SDFE$.
\begin{description}
\item[$\Setup(1^\secp)\ra(\pk,\msk)$:] The setup algorithm takes a security parameter $1^\secp$, and outputs a public key $\pk$ and a master secret key $\msk$.
%\item The key generation algorithm $\KG$, given a master secret key $\msk$ and a function $f\in \cF$, outputs a functional decryption key $\sk_f$.
\item[$\QKeyGen(\msk,f)\ra\qsk_f$:] The key generation algorithm takes a master secret key $\msk$ and a function $f\in\cF$, and outputs a quantum functional decryption key $\qsk_f$.
\item[$\Enc(\pk,x)\ra\ct$:] The encryption algorithm takes a public key $\pk$ and a plaintext $x \in \cX$, and outputs a ciphertext $\ct$.
\item[$\qDec(\qsk_f,\ct)\ra y$:] The decryption algorithm takes a quantum functional decryption key $\qsk_f$ and a ciphertext $\ct$, and outputs $y \in \{ \bot \} \cup \cY$.

\item[Correctness:] For every $\secp\in \bbN$, $x \in \cX$, $f \in \cF$, $(\pk,\msk)$ in the support of $\Setup(1^\secp)$,
we require that
\[\qDec(\QKeyGen(\msk,f), \Enc(\pk,x)) \allowbreak = f(x).\]
\end{description}
\end{definition}

Note that $\Setup$ and $\Enc$ are classical algorithms as~\cref{def:single_dec_PKE}.

\begin{definition}[Adaptive Security for SDFE]\label{def:adaptive_SDFE}
We say that $\SDFE$ is an \emph{adaptively secure} SDFE scheme for $\Xs,\Ys$, and $\Fs$, if it satisfies the following requirement, formalized from the experiment $\expb{\SDFE,\qA}{ada}{ind}(1^\secp,\coin)$ between an adversary $\qA$ and a challenger:
        \begin{enumerate}
            % \item $\qA$ submits a message pair $x_0^*,x_1^* \in \Ms$
            % to the challenger.
            \item The challenger runs $(\pk,\msk)\gets\Setup(1^\secp)$ and sends $\pk$ to $\qA$.
            \item $\qA$ sends arbitrary key queries. That is, $\qA$ sends function $f_{i}\in\Fs$ to the challenger and the challenger responds with $\qsk_{f_{i}}\gets\QKeyGen(\msk,f_i)$ for the $i$-th query $f_{i}$.
            \item At some point, $\qA$ sends $(x_0,x_1)$ to the challenger. If $f_i(x_0)=f_i(x_1)$ for all $i$, the challenger generates a ciphertext $\ct^*\gets\Enc(\pk,x_\coin)$. The challenger sends $\ct^*$ to $\qA$.
            \item Again, $\qA$ can sends function queries $f_i$ such that $f_i(x_0)=f_i(x_1)$.
            \item $\qA$ outputs a guess $\coin^\prime$ for $\coin$.
            \item The experiment outputs $\coin^\prime$.
% if $f_i(m_0^*) = f_i(m_1^*)$ for all $i\in [q_k]$ and $\bot$ otherwise.
        \end{enumerate}
        We say that $\SDFE$ is adaptively secure if, for any QPT $\qA$, it holds that
\begin{align}
%\adva{\A}{sel} \set \Pr\left[\expt{A}{sel} (1^\secp,0)=1\right] - \Pr\left[\expt{\A}{sel}(1^\secp,1)=1\right] \leq \mu(\secp).
\advb{\SDFE,\qA}{ada}{ind}(\secp) \seteq \abs{\Pr[\expb{\SDFE,\qA}{ada}{ind} (1^\secp,0) \out 1] - \Pr[\expb{\SDFE,\qA}{ada}{ind} (1^\secp,1) \out 1] }\leq \negl(\secp).
\end{align}
If $\qA$ can send only one key query during the experiment, we say $\SDFE$ is adaptively single-key secure.
\end{definition}




\begin{definition}[Testing a Quantum FE Distinguisher]\label{def:test_quantum_decryptor_FE}
Let $\gamma \in [0,1]$. Let $\pk$, $(x_0,x_1)$, and $f^\ast$ be a public key, a pair of plaintexts, and a function respectively such that $f^\ast(x_0)\ne f^\ast(x_1)$.
A test for a $\gamma$-good quantum FE distinguisher with respect to $\pk$, $(x_0,x_1)$, and $f^\ast$ is the following procedure.
\begin{itemize}
\item The procedure takes as input a quantum FE decryptor $\pirateD =(\qstateq,\mat{U})$.
\item Let $\cP = (\mat{P}, \mat{I} - \mat{P})$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
\begin{itemize}
\item Sample a uniformly random $\coin\chosen \bit$ and compute $\ct \gets \Enc(\pk,x_\coin)$.
% \item Run $y^\prime \gets \pirateD(\ct)$. If $y^\prime = f^\ast(x_\coin)$, output $1$, otherwise output $0$.
\item Run $\coin^\prime \gets \pirateD(\ct)$. If $\coin^\prime = \coin$, output $1$; otherwise output $0$.
\end{itemize}
Let $\TI_{1/2+\gamma}(\cP)$ be the threshold implementation of $\cP$ with threshold $\frac{1}{2}+\gamma$.
Apply $\TI_{1/2+\gamma}(\cP)$ to $\qstateq$. If the outcome is $1$, we say that the test passed, otherwise the test failed.
\end{itemize}
\end{definition}
We follow the spirit of~\cref{def:test_quantum_decryptor_rand_msg}. That is, we consider a quantum distinguisher rather than a quantum decryptor that computes $f^\ast(x_\coin)$.

% \begin{corollary}[$\gamma$-good Distinguisher for FE]\label{cor:good_dec_FE}
% \fuyuki{We do not need this? We discussed that \cite{C:CLLZ21} needed this corollary for extraction.}
% Let
% \begin{itemize}
% \item $\gamma \in [0,1]$
% \item $(\qstateq,\mat{U})$ be a quantum FE decryptor
% \item $\TI_{1/2 + \gamma}(\cP)$ be the test for a $\gamma$-good FE distinguisher defined in~\cref{def:test_quantum_decryptor_FE}.
% \end{itemize}
% We refer to states which are in the span of all eigenvectors of $\mat{P}$ with eigenvalues at least $1/2+\gamma$ as a $\gamma$-good FE distinguisher with respect to $\pk$, $(x_0,x_1)$, and $f^\ast$. Note that $\cP=(\mat{P},\mat{I}-\mat{P})$.
% Then, the post-measurement state conditioned on output $1$ is a mixture of $\gamma$-good FE decryptor with respect to $\pk$, $(x_0,x_1)$, and $f^\ast$.
% \end{corollary}



\begin{definition}[Strong Anti-Piracy Security for FE]\label{def:strong_anti-piracy_FE}
Let $\gamma \in [0,1]$.
We consider the strong $\gamma$-anti-piracy game $\expc{\SDFE,\qA}{strong}{anti}{piracy}(\secp,\gamma(\secp))$ between the challenger and an adversary $\qA$ below.
\begin{enumerate}
\item The challenger generates $(\pk,\msk)\gets \Setup(1^\secp)$ and sends $\pk$ to $\qA$.
\item $\qA$ sends key queries $f_i$ to the challenger and receives $\qsk_{f_i} \lrun \QKeyGen(\msk,f_i)$.
\item At some point $\qA$ sends a challenge query $f^*$ to the challenger and receives $\qsk_{f^*} \lrun \QKeyGen(\msk,f^*)$.
\item Again, $\qA$ sends $f_i$ to the challenger and receives $\qsk_{f_i} \lrun \QKeyGen(\msk,f_i)$.
\item $\qA$ outputs $(x_0,x_1)$ and two (possibly entangled) quantum decryptors $\pirateD_1 = (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2 = (\qstateq[\qreg{R}_2],\mat{U}_2)$, where $\forall i\ f_i(x_0)=f_i(x_1)$, $f^*(x_0)\ne f^*(x_1)$, $\qstateq$ is a quantum state over registers $\qreg{R}_1$ and $\qreg{R}_2$, and $\mat{U}_1$ and $\mat{U}_2$ are general quantum circuits.
\item The challenger runs the test for a $\gamma$-good FE distinguisher with respect to $\pk$, $(x_0,x_1)$, and $f^\ast$ on $\pirateD_1$ and $\pirateD_2$.
The challenger outputs $1$ if both tests pass, otherwise outputs $0$.
\end{enumerate}

We say that $\SDFE$ is strong $\gamma$-anti-piracy secure if for any QPT adversary $\qA$, it satisfies that
\[
\advc{\SDFE,\qA}{strong}{anti}{piracy}(\secp,\gamma(\secp)) \seteq \Pr[\expc{\SDFE,\qA}{strong}{anti}{piracy}(\secp,\gamma(\secp))=1]  \le  \negl(\sep).
\]
If $\qA$ can send only the challenge query $f^\ast$ during the experiment, we say that $\SDFE$ is challenge-only strong $\gamma$-anti-piracy secure.
\end{definition}
If a pirate has $\qsk_{f^\ast}$, it can easily compute $f^\ast(x_\coin)$ and is a good FE distinguisher since $f^\ast(x_0)\ne f^\ast(x_1)$.
The definition says either $\pirateD_1$ or $\pirateD_2$ do not have the power of $\qsk_{f^\ast}$.

\paragraph{Other security notions for SDFE.}
We can define CPA-style anti-piracy security for SDFE as SDE. We provide the CPA-style anti-piracy security for SDFE in~\cref{def:anti-piracy_CPA_FE}.
We can also define anti-piracy security with random challenge plaintexts for SDFE. However, if we allow adversaries to select a constant-valued function as $f^\ast$, the security is trivially broken. It might be plausible to define security with random challenge plaintexts for functions with high min-entropy. It limits supported classes of functions. However, we focus on FE for all circuits in this work. We omit the definition of anti-piracy with random challenge plaintexts.

\subsection{Single-Key Secure Single-Decryptor Functional Encryption}\label{sec:const_1key_SDFE}

We use the following tools:
\begin{itemize}
\item A single-decryptor encryption $\SDE=(\SDE.\Setup, \SDE.\QKeyGen, \SDE.\Enc, \SDE.\qDec)$.
\item An adaptively secure single-key PKFE scheme $\PKFE=(\PKFE.\Setup,\PKFE.\KG,\allowbreak\PKFE.\Enc,\PKFE.\Dec)$.
\end{itemize}

The description of $\oneSDFE$ is as follows.
\begin{description}

 \item[$\oneSDFE.\Setup(1^\secp)$:] $ $
 \begin{itemize}
 \item Generate $(\fe.\pk,\fe.\msk)\gets \PKFE.\Setup(1^\secp)$.
 \item Generate $(\sde.\pk,\sde.\dk)\gets \SDE.\Setup(1^\secp)$.
 \item Output $\pk \seteq (\fe.\pk,\sde.\pk)$ and $\msk \seteq (\fe.\msk,\sde.\dk)$.
 \end{itemize}
 \item[$\oneSDFE.\QKeyGen(\msk,f)$:] $ $
 \begin{itemize}
 \item Parse $\msk =(\fe.\msk,\sde.\dk)$.
 \item Generate $\fe.\sk_f \gets \PKFE.\KG(\msk,f)$.
 \item Generate $\sde.\qdk \gets\SDE.\QKeyGen(\sde.\dk)$.
 \item Output $\qsk_f \seteq (\fe.\sk_f,\sde.\qdk)$.
 \end{itemize}
 \item[$\oneSDFE.\Enc(\pk,x)$:] $ $
 \begin{itemize}
 \item Parse $\pk = (\fe.\pk,\sde.\pk)$.
 \item Generate $\fe.\ct_x \gets \PKFE.\Enc(\fe.\pk,x)$.
 \item Generate $\sde.\ct \gets \SDE.\Enc(\sde.\pk,\fe.\ct_x)$.
 \item Output $\ct \seteq \sde.\ct$.
 \end{itemize}
\item[$\oneSDFE.\qDec(\qsk_f,\ct)$:] $ $
\begin{itemize}
\item Parse $\qsk_f =(\fe.\sk_f,\sde.\qdk)$ and $\ct = \sde.\ct$.
\item Compute $\fe.\ct_x^\prime\gets\SDE.\qDec(\sde.\qdk,\sde.\ct)$.
\item Output $y\gets\PKFE.\Dec(\fe.\ct_x^\prime)$.
\end{itemize}
\end{description}


\begin{theorem}\label{thm:1SDFE_from_1FE}
If $\PKFE$ is adaptively single-key indistinguishability-secure, $\oneSDFE$ is adaptively single-key secure.
\end{theorem}
\begin{proof}
Suppose that $\advb{\oneSDFE,\qA}{ada}{ind}(\secp)$ is non-negligible for a contradiction.
We construct a QPT algorithm $\qB$ for the adaptive single-key security of $\PKFE$ by using the adversary $\qA$ of the adaptive single-key security game of $\oneSDFE$ as follows.
\begin{enumerate}
\item $\qB$ receives $\fe.\pk$ from its challenger, generates $(\sde.\pk,\sde.\dk)\gets \SDE.\Setup(1^\secp)$, and sends $\pk \seteq(\fe.\pk,\sde.\pk)$ to $\qA$.
\item When $\qA$ sends a key query $f$, $\qB$ sends it to its challenger, receives $\fe.\sk_{f} \gets \PKFE.\KG(\fe.\msk,f)$, computes $\sde.\qdk \gets \SDE.\QKeyGen(\sde.\dk)$, and passes $\qsk_{f} \seteq (\fe.\sk_{f},\sde.\qdk)$ to $\qA$.
\item When $\qA$ sends a pair $(x_0,x_1)$, $\qB$ passes $(x_0,x_1)$ to its challenger and receives $\fe.\ct^\ast \gets \PKFE.\Enc(\fe.\pk,x_\coin)$. $\qB$ generates $\sde.\ct \gets \SDE.\Enc(\sde.\pk,\fe.\ct^\ast)$ and passes $\sde.\ct$ to $\qA$.
\item If $f(x_0)\ne f(x_1)$, $\qB$ aborts. Otherwise, go to the next step.
\item $\qB$ outputs whatever $\qA$ outputs.
\end{enumerate}
It is easy to see that $\qB$ perfectly simulates $\expb{\oneSDFE,\qA}{ada}{ind}(\secp)$ since $\qA$ must send $(f,x_0,x_1)$ such that $f(x_0)=f(x_1)$ due to the condition of $\expb{\oneSDFE,\qA}{ada}{ind}(\secp)$. Thus, $\qB$ breaks the adaptive single-key security of $\PKFE$ by using the distinguishing power of $\qA$. This is a contradiction and we finished the proof.
\end{proof}

\begin{theorem}\label{thm:1SDFE_anti-piracy_from_SDE}
If $\SDE$ is strong $\gamma/4$-anti-piracy secure for randomized function family, $\oneSDFE$ is challenge-only strong $\gamma$-anti-piracy secure.
\end{theorem}

\begin{proof}
We recall the original game.
\begin{description}
\item[$\hybi{0}$:] This is the same as $\expc{\qA,\oneSDFE}{strong}{anti}{piracy}(\secp,\gamma(\secp))$. The detailed description is as follows.
\begin{enumerate}
\item Compute $(\fe.\pk,\fe.\msk) \gets \PKFE.\Setup(1^\secp)$ and $(\sde.\pk,\sde.\dk)\gets\SDE.\Setup(1^\secp)$. Set $\pk \seteq (\fe.\pk,\sde.\pk)$ and $\msk \seteq (\fe.\msk,\sde.\dk)$.
\item Compute $\fe.\sk_{f^\ast} \gets \PKFE.\KG(\fe.\msk,f^\ast)$ and $\sde.\qdk \gets \SDE.\QKeyGen(\sde.\dk)$, and  send $\qsk_{f^\ast} \seteq (\fe.\sk_{f^\ast},\sde.\qdk)$ to $\qA$.
\item Receive $(x_0,x_1)$, $\pirateD_1 =(\qstateq[\qreg{R}_1],\mat{U}_1)$, and $\pirateD_2 =(\qstateq[\qreg{R}_2],\mat{U}_2)$, where $f^\ast(x_0)\ne f^\ast(x_1)$.
\item For $i\in \setbk{1,2}$, let $\cP_{i,D}$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
\begin{itemize}
\item Sample a uniform $\coin \chosen \bit$. Compute $\fe.\ct \gets \PKFE.\Enc(\fe.\pk,x_\coin)$ and $\sde.\ct \gets \SDE.\Enc(\sde.\pk,\fe.\ct)$ and set $\ct \seteq \sde.\ct$.
\item Run the quantum decryptor $(\qstateq^\prime,\mat{U}_i)$ on input $\ct$. If the outcome is % $f^\ast(x_\coin)$,
$\coin$, output $1$. Otherwise, output $0$.
\end{itemize}
Let $D$ be the distribution over pairs $(\coin,\ct)$ defined in the first item above, and let $\cE_i = \setbk{\mat{E}^i_{(\coin,\ct)}}_{\coin,\ct}$ be a collection of projective measurements where $\mat{E}^i_{(\coin,\ct)}$ is the projective measurement described in the second item above.
$\cP_{i,D}$ is the mixture of projective measurements associated to $D$ and $\cE_i$.
\item Run $\TI_{\frac{1}{2}+\gamma}(\cP_{i,D})$ for $i\in \setbk{1,2}$ on quantum decryptor $\pirateD_1=(\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2=(\qstateq[\qreg{R}_2],\mat{U}_2)$.
Output $1$ if both tests pass, otherwise output $0$.
\end{enumerate}
\end{description}

We prove the following.
\begin{lemma}\label{lem:1SDFE_hyb1}
If $\SDE$ is strong $\gamma$-anti-piracy secure with randomized function family $\setbk{\PKFE.\Enc(\fe.\pk,\cdot;\cdot)}_{\secp}$, it holds that $\advc{\SDFE,\qA}{strong}{anti}{piracy}(\secp,\gamma(\secp)) \le \negl(\secp)$.
\end{lemma}
\begin{proof}[Proof of~\cref{lem:1SDFE_hyb1}]
Suppose that $\advc{\SDFE,\qA}{strong}{anti}{piracy}(\secp,\gamma(\secp))$ is non-negligible for a contradiction.
We construct a QPT algorithm $\qB$ for the strong $\gamma$-anti-piracy game with randomized function $\setbk{\PKFE.\Enc(\fe.\pk,\cdot;\cdot)}_{\secp}$ of $\SDE$ by using the adversary $\qA$ of the strong $\gamma$-anti-piracy game of $\SDFE$ as follows.
\begin{enumerate}
\item $\qB$ receives $\sde.\pk$ and $\sde.\qdk$ from its challenger.
\item $\qB$ generates $(\fe.\pk,\fe.\msk) \gets \PKFE.\Setup(1^\secp)$, sets $\pk\seteq (\fe.\pk,\sde.\pk)$, and sends it to $\qA$.
\item When $\qA$ sends the challenge query $f^\ast$, $\qB$ generates $\fe.\sk_{f^\ast} \gets \PKFE.\KG(\fe.\msk,f^\ast)$, sets $\qsk_{f^\ast} \seteq (\fe.\sk_{f^\ast},\sde.\qdk)$, and sends $\qsk_{f^\ast}$ to $\qA$.
\item At some point, $\qB$ receives $(x_0,x_1)$ and two (possibly entangled) quantum decryptors $\pirateD_1 = (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2 = (\qstateq[\qreg{R}_2],\mat{U}_2)$, where $f^*(x_0)\ne f^*(x_1)$, from $\qA$.
\item $\qB$ sets quantum decryptors $\pirateD_1^\ast$ and $\pirateD_2^\ast$ as follows.
$\qB$ sets $\pirateD_1^\ast \seteq (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2^\ast \seteq (\qstateq[\qreg{R}_2],\mat{U}_2)$.
$\qB$ sets a randomized function $g(\cdot;\cdot)\seteq \PKFE.\Enc(\fe.\pk,\cdot;\cdot)$ and sends $(x_0,x_1,g))$ and $\pirateD_1^\ast = (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2^\ast = (\qstateq[\qreg{R}_2],\mat{U}_2)$ to its challenger.
\end{enumerate}
% By the condition $f^\ast(x_0) \ne f^\ast(x_1)$, it holds that $x_0 \ne x_1$.
% By the perfect correctness of $\PKFE$, $\PKFE.\Enc(\fe.\pk,\cdot;\cdot)$ is an injective randomized function.\footnote{If $\Enc(\fe.\pk,x_0;r_0)= \Enc(\fe.\pk,x_1;r_1)$ holds for some $r_0,r_1$, we obtain $f^\ast(x_0)=\Dec(\fe.\sk_{f^\ast},\Enc(\fe.\pk,x_0;r_0)) = \Dec(\fe.\sk_{f^\ast},\Enc(\fe.\pk,x_1;r_1))=f^\ast(x_1)$. This contradicts to $f^\ast(x_0)\ne f^\ast(x_1)$.}
Recall that, for testing quantum decryptors $\pirateD_1$ and $\pirateD_2$ in $\advc{\SDFE,\qA}{strong}{anti}{piracy}(\secp,\gamma(\secp))$, we use the following: For $i\in \setbk{1,2}$, let $\cP_{i,D}$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
\begin{itemize}
\item Sample a uniform $\coin \chosen \bit$. Compute $\fe.\ct \gets \PKFE.\Enc(\fe.\pk,x_\coin)$ and $\sde.\ct \gets \SDE.\Enc(\sde.\pk,\fe.\ct)$ and set $\ct \seteq \sde.\ct$.
\item Run the quantum decryptor $(\qstateq^\prime,\mat{U}_i)$ on input $\ct$. If the outcome is % $f^\ast(x_\coin)$,
$\coin$, output $1$. Otherwise, output $0$.
\end{itemize}

The challenger of $\SDE$ runs the test by using the following.
Let $\cP_{i,D^\prime}$ be the following mixture of projective measurements acting on some quantum state $\qstateq_{\SDE}$:
\begin{itemize}
\item Sample a uniformly random $\coin\chosen \bit$ and $r \chosen \cR$, and compute $m_\coin^\prime \seteq \PKFE.\Enc(\fe.\pk,x_\coin;r)$. Note that $\qB$ sets $g(\cdot,\cdot) \seteq \PKFE.\Enc(\fe.\pk,\cdot;\cdot)$. Then, compute $\ct \gets \SDE.\Enc(\sde.\pk,m_\coin^\prime)$.
\item Run $\coin^\prime \gets \pirateD(\ct)$. If $\coin^\prime = \coin$, output $1$, otherwise output $0$.
\end{itemize}
The distribution is the same as $D$, which $\qB$ simulates. 
% By the injectivity, it holds that for all $r_0,r_1 \in \cR$, $\PKFE.\Enc(\fe.\pk,x_0;r_0) \ne \PKFE.\Enc(\fe.\pk,x_1;r_1)$.

We assumed that $\advc{\SDFE,\qA}{strong}{anti}{piracy}(\secp,\gamma(\secp))$ is non-negligible at the beginning of this proof.
That is, applying $\TI_{\frac{1}{2}+\gamma}(\cP_{i,D})$ on $\qstateq[\qreg{R}_i]$ results in two outcomes $1$ with non-negligible probability:
% By the second item of~\cref{lem:ATI_bipartite_app}, it holds that
\begin{align}
\Tr[\TI_{\frac{1}{2}+\gamma }(\cP_{1,D}) \tensor \TI_{\frac{1}{2}+\gamma }(\cP_{2,D})\qstateq] > \negl(\secp),
\end{align}
where $\mu >\negl(\secp)$ means $\mu$ is non-negligible.
This means that $\qstateq[\qreg{R}_i]$ is a $\gamma$-good distinguisher with respect to ciphertexts generated according to $D$.
It is easy to see that $(\pirateD_1^\ast,\pirateD_2^\ast)$ is a $\gamma$-good distinguisher for randomized function $\PKFE.\Enc(\fe.\pk,\cdot;\cdot)$ since $D^\prime$ and $D$ are the same distribution.
Thus, if $\qA$ outputs $\gamma$-good distinguisher, $\qB$ can also outputs $\gamma$-good distinguisher for randomized function $\PKFE.\Enc(\fe.\pk,\cdot;\cdot)$. This completes the proof of~\cref{lem:1SDFE_hyb1}.
\end{proof}
By~\cref{lem:1SDFE_hyb1}, we complete the proof of~\cref{thm:1SDFE_anti-piracy_from_SDE}.
\end{proof}


We obtain the following corollary from~\cref{thm:SDE_rand_from_IO_LWE,thm:1SDFE_from_1FE,thm:1SDFE_anti-piracy_from_SDE}.

\begin{corollary}\label{cor:strong_1SDFE_from_IO_LWE}
Assuming the existence of sub-exponentially secure IO for $\Ppoly$ and OWFs, and the hardness of QLWE, there exists an SDFE scheme for $\Ppoly$ that satisfies adaptive single-key security and challenge-only strong $\gamma$-anti-piracy security for any inverse polynomial $\gamma$.
\end{corollary}



\begin{remark}[On approximation version of threshold implementation]\label{remark:on_ATI}
We do not need to use approximate version of $\TI$ that runs in polynomial time (denoted by $\ATI$ by previous works~\cite{C:ALLZZ21,C:CLLZ21}) because we do not extract information from pirate decryptors $\pirateD_1$ and $\pirateD_2$.
We use the decision bits output by them for breaking the security of cryptographic primitives in security reductions.
This is the same for the construction in~\cref{sec:const_multi-key_SDFE}.
\end{remark}
\subsection{Collusion-Resistant Single-Decryptor Functional Encryption}\label{sec:const_multi-key_SDFE}
\begin{construction}
We use the following tools:
\begin{itemize}
\item A single-key SDFE $\oneSDFE=(\oneSDFE.\Setup,\oneSDFE.\KG, \oneSDFE.\QKeyGen, \oneSDFE.\Enc,\allowbreak \oneSDFE.\qDec)$.
\item An IO $\iO$.
\item A puncturable PRF $\PuncPRF=(\prfgen,\prf,\Puncture)$, where $\prf: \zo{\secp}\times \zo{\ell} \ra \cR_{\Setup}$ and $\cR_{\Setup}$ is the randomness space of $\oneSDFE.\Setup$.
\item A puncturable PRF $\PuncPRF^\prime=(\prfgen^\prime,\prf^\prime,\Puncture^\prime)$, where $\prf^\prime: \zo{\secp}\times \zo{\ell} \ra \cR_{\Enc}$ and $\cR_{\Enc}$ is the randomness space of $\oneSDFE.\Enc$.
\item A (standard) PRF $\prf^{(1)}: \zo{\secp}\times \cC_{\oneSDFE} \ra \cR_{\prfgen^\prime}$, $\cC_{\oneSDFE}$ is the ciphertext space of $\oneSDFE$ and $\cR_{\prfgen^\prime}$ is the randomness space of $\prfgen^\prime$.
\item A (standard) PRF $\prf^{(2)}: \zo{\secp}\times \cC_{\oneSDFE} \ra \cR_{\iO}$, $\cC_{\oneSDFE}$ is the ciphertext space of $\oneSDFE$ and $\cR_{\iO}$ is the randomness space of $\iO$.
\end{itemize}
Note that we use $\prf^{(1)}$ and $\prf^{(2)}$ only in security proofs.

\begin{description}
\item[$\SDFE.\Setup(1^\secp)$:] $ $
\begin{itemize}
\item Generate $\prfkey \gets \prfgen(1^\secp)$ and $\sfS_{\sfonefe}[\prfkey]$ defined in~\cref{fig:setup-pkfe}.
\item Return $(\pkhat ,\mskhat) \seteq (\iO_1(\sfS_{\sfonefe}),\prfkey)$.
\end{itemize}

\item[$\SDFE.\QKeyGen(\mskhat,f)$:] $ $
\begin{itemize}
\item Parse $\prfkey = \mskhat$ and choose $\gtag \chosen \zo{\ell}$.
\item Compute $r_{\gtag} \gets \prf_{\prfkey}(\gtag)$ and $(\msk_{\gtag}, \pk_{\gtag}) \gets \oneSDFE.\Setup(1^\secp; r_{\gtag})$.
\item Generate $\qsk_{f,\gtag} \gets \oneSDFE.\QKeyGen(\msk_{\gtag},f)$.
\item Output $\qskhat_{f,\gtag} \seteq (\gtag,\qsk_{f,\gtag})$.
\end{itemize}
\item[$\SDFE.\Enc(\pkhat, x)$:] $ $
\begin{itemize}
\item Generate $\prfkey^\prime \gets \prfgen^\prime(1^\secp)$ and $\sfE_\sfonefe[\pkhat,\prfkey^\prime,x]$ defined in~\cref{fig:enc-one-pkfe}.
\item Return $\cthat \gets \iO_2(\sfE_\sfonefe[\pkhat,\prfkey^\prime,x])$.
\end{itemize}

\item[$\SDFE.\qDec(\qskhat_f, \cthat)$:] $ $
\begin{itemize}
\item Parse $(\gtag, \qsk_{f,\gtag}) = \qskhat_f$.
\item Evaluate the circuit $\cthat$ on input $\gtag$, that is $\ct_{\gtag} \gets \cthat(\gtag)$.
\item Return $y \gets \oneSDFE.\qDec(\qsk_{f,\gtag}, \ct_{\gtag})$.
\end{itemize}
\end{description}
 \end{construction}

\protocol
{Setup Circuit $\sfS_{\sfonefe} [\prfkey](\gtag)$}
{Description of $\sfS_{\sfonefe} [\prfkey]$.}
{fig:setup-pkfe}
{
\ifnum\llncs=1
\scriptsize
\else
\fi
\begin{description}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item[Hardwired:] puncturable PRF key $\prfkey$.
\item[Input:] tag $\gtag \in \zo{\ell}$.
\item[Padding:] circuit is padded to size $\padsize_\sfS \seteq \padsize_{\sfS} (\secp,n,s,\ell)$, which is determined in analysis.
\end{description}
\begin{enumerate}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item Compute $r_\gtag \gets \prf_{\prfkey}(\gtag)$.
\item Compute $(\pk_{\gtag}, \msk_{\gtag}) \gets \oneSDFE.\Setup(1^\secp;r_{\gtag})$ and output $\pk_{\gtag}$.
\end{enumerate}
}
\ifnum\llncs=1
\vspace{-5mm}
\else
\fi

\protocol
{Encryption Circuit $\sfE_\sfonefe[\pkhat,\prfkey^\prime, x](\gtag)$}
{Description of $\sfE_\sfonefe[\pkhat,\prfkey^\prime, x]$.}
{fig:enc-one-pkfe}
{
\ifnum\llncs=1
\scriptsize
\else
\fi
\begin{description}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item[Hardwired:] circuit $\pkhat$, puncturable PRF key $\prfkey^\prime$, and message $x$.
\item[Input:] tag $\gtag \in \zo{\ell}$.
\item[Padding:] circuit is padded to size $\padsize_{\sfE} \seteq \padsize_{\sfE}(\secp,n,s,\ell)$, which is determined in analysis.
\end{description}
\begin{enumerate}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item Evaluate the circuit $\pkhat$ on input $\gtag$, that is $\pk_{\gtag} \gets \pkhat(\gtag)$.
\item Compute $r_{\gtag}^\prime \gets \prf^\prime_{\prfkey^\prime}(\gtag)$ and output $\ct_{\gtag} \gets \oneSDFE.\Enc(\pk_{\gtag},x;r^\prime_{\gtag})$.
\end{enumerate}
}

\ryo{OLD PROOF.}
\begin{theorem}\label{thm:SDFE_from_1FE_IO}
If $\oneSDFE$ is adaptively single-key secure, $\iO$ is a secure IO for $\Ppoly$, and $\PuncPRF$ is a PPRF, $\SDFE$ is adaptively secure.
\end{theorem}
\begin{proof}
We define a sequence of hybrid games.
For the hybrid games, we present some definitions.
Let $q$ be the total number of key queries by $\qA$. Note that $q$ could be any polynomial.
When we start the adaptive security game, the adversary $\qA$ is fixed, and $q$ is also fixed. We choose tags $\gtag_1,\ldots,\gtag_q \chosen \zo{\ell}$ for $q$ key queries at the beginning of the game.
We can sort these tags in the ascending order $\gtag_{j_1}<  \cdots < \gtag_{j_{q}}$ where $j_i \in [q]$.
We can interpret $\ell$ bit strings as integers and assume that there is no $i,j$ such that $i\ne j$ and $\gtag_i = \gtag_j$ without loss of generality.
We rename $\gtag^\prime_{i} \seteq \gtag_{j_i}$. It trivially holds that $\gtag^\prime_{1}<  \cdots < \gtag^\prime_{q}$.
Our reduction algorithm can identify which $\gtag^\prime_i$ should be used when it receives the $k$-th query since it can have a permutation $\pi$ such that $\gtag^\prime_{\pi(k)} = \gtag_{k}$.

\begin{description}
\item[$\hybi{0}(\coin)$:] This is the original adaptive security game.
\begin{enumerate}
\item The challenger generates $(\pkhat,\mskhat)=(\iO_1(\sfS_\sfonefe),\prfkey)\gets \SDFE.\Setup(1^\secp)$ and sends $\pkhat$ to $\qA$.
\item $\qA$ sends key queries $f_k$ to the challenger and the challenger generates $r_{\gtag_k} \gets \prf_\prfkey(\gtag_k)$ and $(\pk_{\gtag_k},\msk_{\gtag_k}) \gets \oneSDFE.\Setup(1^\secp;r_{\gtag_k})$, and returns $\qskhat_{f_k} = (\gtag_k,\qsk_{f_k,\gtag_k})$ where $\qsk_{f_k,\gtag_k}\lrun \oneSDFE.\QKeyGen(\msk_{\gtag_k},f_k)$.
\item At some point $\qA$ sends a pair $(x_0,x_1)$ to the challenger.
If $f_i(x_0)=f_i(x_1)$, the challenger generates $\prfkey^\prime \gets \prfgen^\prime(1^\secp)$ and $\sfE_\sfonefe[\pkhat,\prfkey^\prime,x]$ defined in~\cref{fig:enc-one-pkfe} and sends $\cthat \gets \iO_2(\sfE_\sfonefe[\pkhat,\prfkey^\prime,x])$ to $\qA$.
\item Again, $\qA$ sends $f_k$ to the challenger and the challenger returns $\qskhat_{f_k} \lrun \SDFE.\QKeyGen(\mskhat,f_k)$ if $f_k(x_0)=f_k(x_1)$.
\item When $\qA$ outputs $\coin^\prime$, the game outputs $\coin^\prime$.
\end{enumerate}

Let $i \in [q]$.
In the following hybrid games, we gradually change $\sfS_\sfonefe$ and $\sfE_\sfonefe$ for the $i$-th tag $\gtag^\prime_i$ such that $\gtag^\prime_1 < \cdots < \gtag^\prime_i < \cdots < \gtag^\prime_q$.
Let $\Adv_{0}(\coin)$ and $\Adv_{x}^{i}$ be the advantage of $\qA$ in $\hybi{0}(\coin)$ and $\hybij{x}{i}$, respectively.

 \item[$\hybij{1}{i}$:] We generate $\pkhat$ as obfuscated $\sfS^*_\sfonefe$ described in~\cref{fig:setup-pkfe-punc}. In this hybrid game, we set $r_{i} \la \prf_{\prfkey}(\gtag^\prime_i)$, $\prf_{\ne \gtag^\prime_i} \la \Puncture(\prfkey,\gtag^\prime_i)$, $(\pk_{\gtag^\prime_i},\msk_{\gtag^\prime_i}) \la \oneSDFE.\Setup(1^\secp ;r_{i})$, and $\pkhat \gets \iO_1(\sfS^\ast_\sfonefe [\gtag^\prime_i,\prf_{\ne \gtag^\prime_i},\pk_{\gtag^\prime_i}])$.

When $i=1$, the behavior of $\sfS^*_\sfonefe$ is the same as that of $\sfS_\sfonefe$ since the hard-wired $\pk_{\gtag^\prime_1}$ in $\sfS^*_\sfonefe$ is the same as the output of $\sfS_\sfonefe$ on the input $\gtag^\prime_1$. Their size is also the same since we pad circuit $\sfS_\sfonefe$ to have the same size as $\sfS_\sfonefe^*$. Then, we can use the indistinguishability of $\iO_1$ and it holds that $\abs{\Adv_{0}(0) - \Adv_{1}^{1}} \le \negl(\secp)$.

\item[$\hybij{2}{i}$:] The challenge ciphertext is generated by obfuscating $\sfE^*_\sfonefe$ described in~\cref{fig:enc-one-pkfe-punc}. In this hybrid game, we set $r^\prime_{i} \la \prf^\prime_{\prfkey^\prime}(\gtag^\prime_i)$, $\prf^\prime_{\ne \gtag^\prime_i} \la \Puncture(\prfkey^\prime,\gtag^\prime_i)$, $\ct_{i} \la \oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_0 ;r'_{i})$, $\pk_{\gtag^\prime_i} \la \pkhat(\gtag^\prime_i)$, and $\cthat \gets \iO_2(\sfE_\sfonefe[\gtag^\prime,\pkhat,\prf^\prime_{\ne \gtag^\prime},\allowbreak x_0,x_1,\ct_{\gtag^\prime}])$.

When $i=1$, the behavior of $\sfE^*_\sfonefe$ is the same as that of $\sfE_\sfonefe$ since the hard-wired $\ct_1$ in $\sfE^*_\sfonefe$ is the same as the output of $\sfE_\sfonefe$ on the input $1$. Both circuits have the same size by padding $\pad_\sfE$.

In addition, for $i \geq 2$, the behavior of $\sfE^*_\sfonefe$ does not change between $\hybij{1}{i}$ and $\hybij{2}{i}$.
Thus, it holds that $\abs{\Adv_{2}^{i}- \Adv_{1}^{i} }\le \negl(\secp)$ for every $i \in [q]$ due to the indistinguishability of $\iO_2$.


\protocol
{Setup Circuit $\sfS^*_{\sfonefe} [\gtag^\prime,\prf_{\ne \gtag^\prime},\pk_{\gtag^\prime}](\gtag)$}
{Description of $\sfS^*_{\sfonefe} [\gtag^\prime,\prf_{\ne \gtag^\prime},\pk_{\gtag^\prime}]$.
}
{fig:setup-pkfe-punc}
{
\ifnum\llncs=1
\scriptsize
\else
\fi
\begin{description}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item[Hardwired:] tag $\gtag^\prime$, puncturable PRF key $\prf_{\ne \gtag^\prime}$, and $\oneSDFE$ public-key $\pk_{\gtag^\prime}$.
\item[Input:] tag $\gtag \in \zo{\ell}$.
\item[Padding:] circuit is padded to size $\padsize_{\sfS}\seteq\padsize_{\sfS}(\secp,n,s)$, which is determined in analysis.
\end{description}
\begin{enumerate}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item If $\gtag^\prime = \gtag$, output $\pk_{\gtag^\prime}$.
\item Else, compute $r \gets \prf_{\ne \gtag^\prime}(\gtag)$.
\item Compute $(\pk_{\gtag}, \msk_{\gtag}) \gets \oneSDFE.\Setup(1^\secp;r)$ and output $\pk_{\gtag}$.
\end{enumerate}
}


\protocol
{Encryption Circuit $\sfE^*_\sfonefe[\gtag^\prime,\pkhat,\prf^\prime_{\ne \gtag^\prime}, x_0,x_1,\ct_{\gtag^\prime}](\gtag)$}
{Description of $\sfE^*_\sfonefe[\gtag^\prime,\pkhat,\prf^\prime_{\ne \gtag^\prime}, x_0,x_1,\ct_{\gtag^\prime}]$.
}
{fig:enc-one-pkfe-punc}
{
\ifnum\llncs=1
\scriptsize
\else
\fi
\begin{description}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item[Hardwired:] tag $\gtag^\prime$, public key $\pkhat$ (this is an obfuscated circuit), puncturable PRF key $\prf^\prime_{\ne \gtag^\prime}$, plaintexts $x_0,x_1$, and ciphertext $\ct_{\gtag^\prime}$.
\item[Input:] tag $\gtag \in \zo{\ell}$.
\item[Padding:] circuit is padded to size $\padsize_{\sfE}\seteq\padsize_{\sfE}(\secp,n,s)$, which is determined in analysis.
\end{description}
\begin{enumerate}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item If $\gtag^\prime = \gtag$, output $\ct_{\gtag^\prime}$.
\item Else, compute $r^\prime_{\gtag} \gets \prf^\prime_{\ne \gtag^\prime}(\gtag)$ and the circuit $\pkhat$ on input $\gtag$, that is, $\pk_{\gtag} \gets \pkhat(\gtag)$,
\begin{description}
\item[If $\gtag > \gtag^\prime$:] Output $\ct_\gtag \gets \oneSDFE.\Enc(\pk_{\gtag},x_0;r^\prime_{\gtag})$.
\item[If $\gtag < \gtag^\prime$:] Output $\ct_\gtag \gets \oneSDFE.\Enc(\pk_{\gtag},x_1;r^\prime_{\gtag})$.
\end{description}
\end{enumerate}
}

\item[$\hybij{3}{i}$:] We change $r_{i} = \prf_{\prfkey}(\gtag^\prime_i)$ and $r^\prime_{i} = \prf^\prime_{\prfkey^\prime}(\gtag^\prime_i)$ into uniformly random $r_{i}$ and $r^\prime_{i}$. Due to the pseudorandomness at punctured points of puncturable PRF, it holds that $\abs{\Adv_{3}^{i}- \Adv_{2}^{i} }\le \negl(\secp)$ for every $i \in [q]$.

\item[$\hybij{4}{i}$:] We change $\ct_{\gtag^\prime_i}$ from $\oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_0)$ to $\oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_1)$.
In $\hybij{3}{i}$ and $\hybij{4}{i}$, we do not need randomness to generate $\pk_{\gtag^\prime_i}$ and $\ct_{\gtag^\prime_i}$.
We just hardwire $\pk_{\gtag^\prime_i}$ and $\ct_{\gtag^\prime_i}$ into $\sfS^*_\sfonefe$ and $\sfE^*_\sfonefe$, respectively. Therefore, for every $i \in [q]$, $\abs{\Adv_{4}^{i}- \Adv_{3}^{i} }\le \negl(\secp)$ follows from the adaptive security of $\oneSDFE$ under the master public key $\pk_{\gtag^\prime_i}$.
\begin{lemma}\label{lem:ind-by-one-pkfe}
It holds that $\abs{\Adv_{4}^{i}- \Adv_{3}^{i} }\le \negl(\secp)$ for all $i \in [q]$ if $\oneSDFE$ is adaptively single-key secure.
\end{lemma}
\begin{proof}[Proof of~\cref{lem:ind-by-one-pkfe}]
We construct an adversary $\qB$ in the selective security game of $\oneSDFE$ as follows. To simulate the adaptive security game of $\SDFE$, $\qB$ runs $\qA$ attacking $\oneSDFE$. $\qA$ adaptively sends key queries $f_1,\cdots,f_q$. $\qB$ simulates the game of $\SDFE$ as follows.
\begin{description}
\item[Setup:] $\qB$ receives a public key $\pk_{\gtag^\prime_i}$. Then, $\qB$ generates $\prfkey$ and $\prfkey^\prime$ by using $\prfgen(1^\secp)$ and $\prfgen^\prime(1^\secp)$, $\prf_{\ne \gtag^\prime_i} \gets \Puncture(\prfkey,\gtag^\prime_i)$, $\prf^\prime_{\ne \gtag^\prime_i} \gets \Puncture(\prfkey^\prime,\gtag^\prime_i)$, and the public key $\pkhat \seteq \iO_1(\sfS^*_\sfonefe[\gtag^\prime_i,\prf_{\ne \gtag^\prime_i},\pk_{\gtag^\prime_i}])$ for $\SDFE$ according to \cref{fig:setup-pkfe-punc} by using the given $\pk_{\gtag^\prime_i}$. $\qB$ sends $\pkhat$ to $\qA$.
\item[Key Generation:] When $f_k$ (i.e., $k$-th query) is queried, $\qB$ checks $f_k(x_0)=f_k(x_1)$ and outputs $\bot$ if it does not hold. Otherwise, $\qB$ computes $\pi(k)$ and reads $\gtag^\prime_{\pi(k)}$. Let $k^\ast \in [q]$ be the index that satisfies $\gtag^\prime_{i}=\gtag_{k^\ast}$ (i.e., $i$-th tag in the ascending order sorted tags). $\qB$ passes $f_{k^\ast}$ to its challenger, receives $\qsk_{f_{k^\ast}}$, and sends $(\gtag^\prime_i,\qsk_{f_{k^\ast}})$ to $\qA$. If $\gtag^{\prime}_i \ne \gtag^\prime_{i^{\prime\prime}} = \gtag_{k} $ (i.e., $k\ne k^\ast$), $\qB$ generates $\qsk_{f_k} \gets \oneSDFE.\QKeyGen (\msk_{\gtag^\prime_{i^{\prime\prime}}},f_k)$ by using $(\pk_{\gtag^\prime_{i^{\prime\prime}}},\msk_{\gtag^\prime_{i^{\prime\prime}}}) \gets \oneSDFE.\Setup(1^\secp;\prf_{\ne \gtag^\prime_{i}}(\gtag^\prime_{i^{\prime\prime}}))$ and returns it. Note that we do not need $\msk_{\gtag^\prime_i}$ for this simulation since $\qB$ receives $\qsk_{f_{k^\ast}}$ from its challenger. 
\item[Encryption:] When $\qA$ sends $(x_0,x_1)$ to $\qB$, $\qB$ passes $(x_0,x_1)$ to its challenger and receives $\ct^\ast_{\gtag^\prime_i}$. Then, $\qB$ generates the challenge ciphertext $\cthat \gets \iO_2(\sfE^\ast[\gtag^\prime_i,\pkhat,\prf^\prime_{\ne \gtag^\prime_{i}},x_0,x_1,\ct^\ast_{\gtag^\prime_i}])$ (obfuscated $\sfE^*_\sfonefe$~\cref{fig:enc-one-pkfe-punc}).
\end{description}
The simulation is completed. If $\qB$ receives $\ct^\ast_{\gtag^\prime_{i}} = \oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_0)$, it perfectly simulates $\hybij{3}{i}$. If $\qB$ receives $\ct^\ast_{\gtag^\prime_i} = \oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_1)$, it perfectly simulates $\hybij{4}{i}$. This completes the proof of the lemma.
\end{proof}
\item[$\hybij{5}{i}$:] We change $r_i$ and $r^\prime_{i}$ into $r_{i} = \prf_{\prfkey}(\gtag^\prime_i)$ and $r^\prime_{i} = \prf^\prime_{\prfkey^\prime}(\gtag^\prime_i)$. We can show $\abs{\Adv_{5}^{i}- \Adv_{4}^{i} }\le \negl(\secp)$ for every $i \in [q]$ by using the pseudorandomness at punctured point of puncturable PRF.
\end{description}
From the definition of $\sfS^*_{\sfonefe}$, $\sfE^*_{\sfonefe}$, and $\hybij{1}{i}$, the behaviors of $\sfS^*_{\sfonefe}$ and $\sfE^*_{\sfonefe}$ in $\hybij{5}{i}$ and $\hybij{1}{i+1}$ are the same. Thus, $\abs{\Adv_{1}^{i+1}- \Adv_{5}^{i} }\le \negl(\secp)$ holds for every $ \in [q-1]$ due to the indistinguishability of $\iO_1$ and $\iO_2$.
It also holds that $\abs{\Adv_{0}(1)- \Adv_{5}^{q} }\le \negl(\secp)$ based on the security guarantee of $\iO_1$ and $\iO_2$.

\paragraph{Padding Parameter.} The proof of security relies on the indistinguishability of obfuscated $\sfS_{\sfonefe}$ and $\sfS^*_{\sfonefe}$ defined in~\cref{fig:setup-pkfe,fig:setup-pkfe-punc},
and that of obfuscated $\sfE_\sfonefe$ and $\sfE_\sfonefe^\ast$ defined in~\cref{fig:enc-one-pkfe,fig:enc-one-pkfe-punc}. Accordingly, we set $\padsize_{\sfS} \seteq \max(\abs{\sfS_{\sfonefe}},\abs{\sfS_{\sfonefe}^*})$ and $\padsize_{\sfE} \seteq \max(\abs{\sfE_{\sfonefe}},\abs{\sfE_{\sfonefe}^*})$.

The circuits $\sfS_\sfonefe$ and $\sfS_\sfonefe^*$ compute a puncturable PRF over domain $\zo{\ell}$ and a key pair of $\oneFE$, and may have punctured PRF keys and a public key hardwired. The circuits $\sfE_\sfonefe$ and $\sfE_\sfonefe^*$ run the circuit $\pkhat$ and compute a puncturable PRF over domain $\zo{\ell}$ and a ciphertext of $\oneSDFE$, and may have punctured PRF keys, tags, plaintexts, and a hard-wired ciphertext. Note that $\ell$ is a polynomial of $\secp$. Thus, it holds that
 \begin{align}
 \pad_{\sfS} & \le \poly(\secp,n,s),\\
 \pad_{\sfE} & \le \poly(\secp,n,s,\abs{\pkhat}).
 \end{align}
 Therefore, we complete the proof of~\cref{thm:SDFE_from_1FE_IO}.
\end{proof}

\begin{theorem}\label{thm:SDFE_anti-piracy_from_1SDFE_IO}
If $\oneSDFE$ is challenge-only strong $\gamma/2$-anti-piracy secure and adaptively single-key secure, $\iO$ is a secure IO for $\Ppoly$, and $\PuncPRF$ and $\PuncPRF^\prime$ are puncturable PRFs, $\SDFE$ is strong $\gamma$-anti-piracy secure.
\end{theorem}

\begin{proof}[Proof of~\cref{thm:SDFE_anti-piracy_from_1SDFE_IO}]
Let $\qA$ be an adversary attacking the strong $\gamma$-anti-piracy of $\SDFE$.
We define a sequence of hybrid games.
For the hybrid games, we define the following values.
Let $q$ be the total number of key queries by $\qA$ except for the challenge query $f^\ast$. Note that $q$ could be any polynomial.
When we start the strong $\gamma$-anti-piracy security game, the adversary $\qA$ is fixed, and $q$ is also fixed. We choose tags $\gtag_1,\ldots,\gtag_q \chosen \zo{\ell}$ for $q$ key queries and $\gtag^\ast$ for the challenge query at the beginning of the game.
We can sort these tags except $\gtag^\ast$ in the ascending order $\gtag_{j_1}<  \cdots < \gtag_{j_{q}}$ where $j_i \in [q]$.
We can interpret $\ell$ bit strings as integers and assume that there is no $i,j$ such that $i\ne j$ and $\gtag_i = \gtag_j$ without loss of generality.
We rename $\gtag^\prime_{i} \seteq \gtag_{j_i}$. It trivially holds that $\gtag^\prime_{1}<  \cdots < \gtag^\prime_{q}$.
Our reduction algorithm can identify which $\gtag^\prime_i$ should be used when it receives the $k$-th query since it can have a permutation $\pi$ such that $\gtag^\prime_{\pi(k)} = \gtag_{k}$.
We also sets $\gtag^\prime_{q+1}\seteq \gtag^\ast$.

\begin{description}
\item[$\hybi{0}$:] The first game is the original strong $\gamma$-anti-piracy experiment, that is, $\expc{\SDFE,\qA}{strong}{anti}{piracy}(1^\secp,\gamma)$.
\begin{enumerate}
\item The challenger generates $(\pkhat,\mskhat)=(\iO_1(\sfS_\sfonefe),\prfkey)\gets \SDFE.\Setup(1^\secp)$ and sends $\pkhat$ to $\qA$.
\item $\qA$ sends key queries $f_k$ to the challenger and the challenger returns $\qskhat_{f_k} = (\gtag_k,\qsk_{f_k,\gtag_k}) \lrun \SDFE.\QKeyGen(\mskhat,f_k)$ where $\qsk_{f_k,\gtag_k}\lrun \oneSDFE.\QKeyGen(\msk_{\gtag_k},f_k)$.
\item At some point $\qA$ sends a challenge query $f^*$ to the challenger and the challenger returns $\qskhat =(\gtag^\ast,\qsk_{f^\ast}) \lrun \SDFE.\QKeyGen(\mskhat,f^\ast)$ where $\qsk_{f^\ast}\lrun \oneSDFE.\QKeyGen(\msk_{\gtag^\ast},f^*)$.
\item Again, $\qA$ sends $f_k$ to the challenger and the challenger returns $\qskhat_{f_k} \lrun \SDFE.\QKeyGen(\mskhat,f_k)$.
\item $\qA$ outputs $(x_0,x_1)$ and two (possibly entangled) quantum decryptors $\pirateD_1 = (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2 = (\qstateq[\qreg{R}_2],\mat{U}_2)$, where $\forall i\ f_i(x_0)=f_i(x_1)$, $f^*(x_0)\ne f^*(x_1)$, $\qstateq$ is a quantum state over registers $\qreg{R}_1$ and $\qreg{R}_2$, and $\mat{U}_1$ and $\mat{U}_2$ are general quantum circuits.
\item For $i\in \setbk{1,2}$, let $\cP_{i,D}$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
\begin{itemize}
\item Sample a uniform $\coin \chosen \bit$. Compute $\cthat \gets \SDFE.\Enc(\pkhat,x_\coin)$ and set $\ct \seteq \cthat$.
\item Run the quantum decryptor $(\qstateq^\prime,\mat{U}_i)$ on input $\ct$. If the outcome is % $f^\ast(x_\coin)$,
$\coin$, output $1$. Otherwise, output $0$.
\end{itemize}
Let $D$ be the distribution over pairs $(\coin,\ct)$ defined in the first item above, and let $\cE_i = \setbk{\mat{E}^i_{(\coin,\ct)}}_{\coin,\ct}$ be a collection of projective measurements where $\mat{E}^i_{(\coin,\ct)}$ is the projective measurement described in the second item above.
$\cP_{i,D}$ is the mixture of projective measurements associated to $D$ and $\cE_i$.
\item The challenger runs the test for a $\gamma$-good FE decryptor with respect to $\pk$, $(x_0,x_1)$, and $f^\ast$ on $\pirateD_1$ and $\pirateD_2$.
The challenger outputs $1$ if both tests pass, otherwise outputs $0$.
\end{enumerate}
Let $\Adv_{x}^{i}$ be the advantage of $\qA$ in $\hybij{x}{i}$.


\item[$\hybij{1}{i}$:] This is defined for $i \in [q+1]$ and the same as $\hybij{5}{i-1}$ except that we generate $\pkhat$ as obfuscated $\sfS^*_\sfonefe$ described in~\cref{fig:setup-sdfe-punc}. Note that we define $\hybij{5}{0}=\hybi{0}$. In this hybrid game, we set $r_{\gtag^\prime_i} \la \prf_{\prfkey}(\gtag^\prime_i)$, $\prf_{\ne \gtag^\prime_i} \la \Puncture(\prfkey,\gtag^\prime_i)$, and $(\pk_{\gtag^\prime_i},\msk_{\gtag^\prime_i}) \la \oneSDFE.\Setup(1^\secp ;r_{\gtag^\prime_i})$.

The behavior of $\sfS^*_\sfonefe$ is the same as that of $\sfS_\sfonefe$ since the hard-wired $\pk_{\gtag^\prime_1}$ in $\sfS^*_\sfonefe$ is the same as the output of $\sfS_\sfonefe$ on the input $\gtag^\prime_1$. Their size is also the same since we pad circuit $\sfS_\sfonefe$ to have the same size as $\sfS_\sfonefe^*$. Then, we can use the indistinguishability guarantee of $\iO_1$ and it holds that $\iO_1(\sfS_\sfonefe[\prfkey])$ is computationally indistinguishable from $\iO_1(\sfS^\ast_\sfonefe[\gtag^\prime_i,\prf_{\ne \gtag^\prime_i},\pk_{\gtag^\prime_i}])$. Let $D^{(1,i)}$ be the distribution over pairs $(\coin,\ct)$ defined in $\hybi{0}$ except that $\iO_1(\sfS^\ast_\sfonefe[\gtag^\prime_i,\prf_{\ne \gtag^\prime_i},\allowbreak\pk_{\gtag^\prime_i}])$ as $\pkhat$. Then, $D^{(1,1)}$ is computationally indistinguishable from $D$.

By~\cref{thm:ind_distribution_TI}, it holds that
\begin{align}
& \Tr[(\TI_{\frac{1}{2}+\gamma -\epsilon}(\cP_{1,D^{(1,1)}}) \tensor \TI_{\frac{1}{2} +\gamma - \epsilon }(\cP_{2,D^{(1,1)}}))\qstateq] \\
& \ge \Tr[(\TI_{D^{},\frac{1}{2}+\gamma }(\cP_{1,D^{}})\tensor \TI_{\frac{1}{2} +\gamma }(\cP_{2,D^{}}))\qstateq] - \delta,
\end{align}
where $\delta$ is some negligible function.
That is, it holds that $ \Adv_{1}^{1} \ge  \Adv_{5}^{0} - \negl(\secp)$.

\item[$\hybij{2}{i}$:] This is defined for $i \in [q+1]$ and the same as $\hybij{1}{i}$ except that we change the distribution $D^{(1,i)}$ over pairs $(\coin,\ct)$ into $D^{(2,i)}$ as follows.
\begin{itemize}
 \item Sample a uniform $\coin \chosen \bit$.
 \item Compute $r^\prime_{\gtag^\prime_i} \la \prf^\prime_{\prfkey^\prime}(\gtag^\prime_i)$, $\prf^\prime_{\ne \gtag^\prime_i} \la \Puncture^\prime(\prfkey^\prime,\gtag^\prime_i)$, $\ct_{\gtag^\prime_i} \la \oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_\coin ;r^\prime_{\gtag^\prime_i})$, and $\cthat \gets \iO_2(\sfE^\ast_\sfonefe[\gtag^\prime_i,\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\prime_i},x_\coin,x_1,\ct_{\gtag^\prime_i}])$ where $\sfE^\ast_\sfonefe$ is described in~\cref{fig:enc-one-sdfe-punc}. Set $\ct \seteq \cthat$.
 \end{itemize} 

\protocol
{Setup Circuit $\sfS^*_{\sfonefe} [\gtag^\prime,\prf_{\ne \gtag^\prime},\pk_{\gtag^\prime}](\gtag)$}
{Circuit $\sfS^*_{\sfonefe} [\gtag^\prime,\prf_{\ne \gtag^\prime},\pk_{\gtag^\prime}]$.
}
{fig:setup-sdfe-punc}
{
\ifnum\llncs=1
\scriptsize
\else
\fi
\begin{description}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item[Hardwired:] tag $\gtag^\prime$, puncturable PRF key $\prf_{\ne \gtag^\prime}$, and $\oneSDFE$ public-key $\pk_{\gtag^\prime}$.
\item[Input:] tag $\gtag \in \zo{\ell}$.
\item[Padding:] circuit is padded to size $\padsize_{\sfS}\seteq\padsize_{\sfS}(\secp,n,s)$, which is determined in analysis.
\end{description}
\begin{enumerate}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item If $\gtag^\prime = \gtag$, output $\pk_{\gtag^\prime}$.
\item Else, compute $r \gets \prf_{\ne \gtag^\prime}(\gtag)$.
\item Compute $(\pk_{\gtag}, \msk_{\gtag}) \gets \oneSDFE.\Setup(1^\secp;r_i)$ and output $\pk_{\gtag}$.
\end{enumerate}
}


\protocol
{Encryption Circuit $\sfE^*_\sfonefe[\gtag^\prime,\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\prime},x_\coin, x_1,\ct_{\gtag^\prime}](\gtag)$}
{Circuit $\sfE^*_\sfonefe[\gtag^\prime,\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\prime},x_\coin,x_1,\ct_{\gtag^\prime}]$.
}
{fig:enc-one-sdfe-punc}
{
\ifnum\llncs=1
\scriptsize
\else
\fi
\begin{description}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item[Hardwired:] tags $\gtag^\prime$, $\gtag^\ast$, public key $\pkhat$ (this is an obfuscated circuit), puncturable PRF key $\prf^\prime_{\ne \gtag^\prime}$, plaintexts $x_\coin,x_1$, and ciphertext $\ct_{\gtag^\prime}$.
\item[Input:] tag $\gtag \in \zo{\ell}$.
\item[Padding:] circuit is padded to size $\padsize_{\sfE}\seteq\padsize_{\sfE}(\secp,n,s)$, which is determined in analysis.
\end{description}
\begin{enumerate}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item If $\gtag^\prime = \gtag$, output $\ct_{\gtag^\prime}$.
\item Else, compute $r^\prime_{\gtag} \gets \prf^\prime_{\ne \gtag^\prime_i}(\gtag)$ and the circuit $\pkhat$ on input $\gtag$, that is, $\pk_{\gtag} \gets \pkhat(\gtag)$,
\begin{description}
    \item[If $\gtag = \gtag^\ast$:] Output $\ct_{\gtag^\ast} \gets \oneSDFE.\Enc(\pk_{\gtag^\ast},x_\coin;r^\prime_{\gtag^\ast})$
\item[If $\gtag > \gtag^\prime$:] Output $\ct_\gtag \gets \oneSDFE.\Enc(\pk_{\gtag},x_\coin;r^\prime_{\gtag})$.
\item[If $\gtag < \gtag^\prime$:] Output $\ct_\gtag \gets \oneSDFE.\Enc(\pk_{\gtag},x_1;r^\prime_{\gtag})$.
\end{description}
% \item Else, compute $r^\prime_{\gtag} \gets \prf_{\prfkey^\prime_{\ne \gtag^\prime}}(\gtag)$ and the circuit $\pkhat$ on input $\gtag$, that is, $\pk_{\gtag} \gets \pkhat(\gtag)$, and output $\ct \gets \oneSDFE.\Enc(\pk_{\gtag},x_\coin;r^\prime_{\gtag})$.
\end{enumerate}
}


The behavior of $\sfE^*_\sfonefe$ is the same as that of $\sfE_\sfonefe$ since the hard-wired $\ct_{\gtag^\prime_i}$ in $\sfE^*_\sfonefe$ is the same as the output of $\sfE_\sfonefe$ on the input $\gtag^\prime_i$.
Moreover, both circuits have the same size by padding $\pad_\sfE$. Then, we can use the indistinguishability of $\iO_2$, and it holds that $D^{(2,i)}$ is computationally indistinguishable from $D^{(1,i)}$.

By~\cref{thm:ind_distribution_TI}, it holds that
\begin{align}
& \Tr[(\TI_{\frac{1}{2}+\gamma -(7i-5)\epsilon}(\cP_{1,D^{(2,i)}}) \tensor \TI_{\frac{1}{2} +\gamma - (7i-5)\epsilon }(\cP_{2,D^{(2,i)}}))\qstateq] \\
& \ge \Tr[(\TI_{\frac{1}{2}+\gamma -(7i-6)\epsilon }(\cP_{1,D^{(1,i)}})\tensor \TI_{\frac{1}{2} +\gamma -(7i-6)\epsilon}(\cP_{2,D^{(1,i)}}))\qstateq] - \delta,
\end{align}
where $\delta$ is some negligible function.
That is, it holds that $\Adv_{2}^{i} \ge  \Adv_{1}^{i}  -\negl(\secp)$.

\item[$\hybij{3}{i}$:] This is defined for $i \in [q+1]$ and the same as $\hybij{2}{i}$ except that we use distribution $D^{(3,i)}$, which is the same as $D^{(2,i)}$ except that setup randomness $r_{\gtag^\ast}\chosen \cR_{\Setup}$ and encryption randomness $r^\prime_{\gtag^\ast}\chosen \cR_{\Enc}$ are uniformly random. By the punctured pseudorandomness of $\prf$ and $\prf^\prime$, $D^{(3,i)}$ is computationally indistinguishable from $D^{(2,i)}$.

By~\cref{thm:ind_distribution_TI}, it holds that
\begin{align}
& \Tr[(\TI_{\frac{1}{2}+\gamma -(7i-3)\epsilon}(\cP_{1,D^{(3,i)}}) \tensor \TI_{\frac{1}{2} +\gamma - (7i-3)\epsilon }(\cP_{2,D^{(3,i)}}))\qstateq] \\
& \ge \Tr[(\TI_{\frac{1}{2}+\gamma -(7i-5)\epsilon }(\cP_{1,D^{(2,i)}})\tensor \TI_{\frac{1}{2} +\gamma -(7i-5)\epsilon }(\cP_{2,D^{(2,i)}}))\qstateq] - 2\delta,
\end{align}
where $\delta$ is some negligible function.
That is, it holds that $\Adv_{3}^{i} \ge  \Adv_{2}^{i} - \negl(\secp)$.
Note that we apply \cref{thm:ind_distribution_TI} twice here since we use punctured pseudorandomness of both $\prf$ and $\prf^\prime$.

\item[$\hybij{4}{i}$:] This is defined for $i \in [q]$ and the same as $\hybij{3}{i}$ except that we use distribution $D^{(4,i)}$, which is the same as $D^{(3,i)}$ except that the ciphertext $\ct_{\gtag^\prime_i}$ is $\oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_1)$ instead of $\oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_\coin)$.
In $\hybij{3}{i}$ and $\hybij{4}{i}$, we do not need randomness to generate $\pk_{\gtag^\prime_i}$ and $\ct_{\gtag^\prime_i}$.
We just hardwire $\pk_{\gtag^\prime_i}$ and $\ct_{\gtag^\prime_i}$ into $\sfS^*_\sfonefe$ and $\sfE^*_\sfonefe$, respectively.
In addition, it holds that $f_k(x_0)=f_k(x_1)$ for all $k\in[q]$ by the requirement of strong $\gamma$-anti-piracy security. For every $i \in [q]$, by the adaptive security of $\oneSDFE$ under the public key $\pk_{\gtag^\prime_i}$, $D^{(4,i)}$ is computationally indistinguishable from $D^{(3,i)}$.
The detail of this indistinguishability is almost the same as~\cref{lem:ind-by-one-pkfe}, and we omit it.

By~\cref{thm:ind_distribution_TI}, it holds that
\begin{align}
& \Tr[(\TI_{\frac{1}{2}+\gamma -(7i-2)\epsilon}(\cP_{1,D^{(4,i)}}) \tensor \TI_{\frac{1}{2} +\gamma - (7i-2)\epsilon }(\cP_{2,D^{(4,i)}}))\qstateq] \\
& \ge \Tr[(\TI_{\frac{1}{2}+\gamma -(7i-3)\epsilon }(\cP_{1,D^{(3,i)}})\tensor \TI_{\frac{1}{2} +\gamma -(7i-3)\epsilon }(\cP_{2,D^{(3,i)}}))\qstateq] - \delta,
\end{align}
where $\delta$ is some negligible function.
That is, it holds that $\Adv_{4}^{i} \ge  \Adv_{3}^{i} - \negl(\secp)$.

\item[$\hybij{5}{i}$:] This is defined for $i\in [q]$ and the same as $\hybij{4}{i}$ except that we use distribution $D^{(5,i)}$, which is the same as $D^{(4,i)}$ except that we use $r_{i} = \prf_{\prfkey}(\gtag^\prime_i)$ and $r^\prime_{i} = \prf^\prime_{\prfkey^\prime}(\gtag^\prime_i)$.
By the punctured pseudorandomness of $\prf$ and $\prf^\prime$, $D^{(5,i)}$ is computationally indistinguishable from $D^{(4,i)}$.

By~\cref{thm:ind_distribution_TI}, it holds that
\begin{align}
& \Tr[(\TI_{\frac{1}{2}+\gamma -(7i)\epsilon}(\cP_{1,D^{(5,i)}}) \tensor \TI_{\frac{1}{2} +\gamma - (7i)\epsilon }(\cP_{2,D^{(5,i)}}))\qstateq] \\
& \ge \Tr[(\TI_{\frac{1}{2}+\gamma -(7i-2)\epsilon }(\cP_{1,D^{(4,i)}})\tensor \TI_{\frac{1}{2} +\gamma -(7i-2)\epsilon }(\cP_{2,D^{(4,i)}}))\qstateq] - 2\delta,
\end{align}
where $\delta$ is some negligible function.

We finish describing one cycle of our hybrid games.
We move from $\hybij{5}{i}$ to $\hybij{1}{i+1}$.
From the definition of $\sfS^*_{\sfonefe}$ and $\hybij{1}{i}$, the behaviors of $\sfS^*_{\sfonefe}$ in $\hybij{5}{i}$ and $\hybij{1}{i+1}$ are the same.
By~\cref{thm:ind_distribution_TI}, it holds that
\begin{align}
& \Tr[(\TI_{\frac{1}{2}+\gamma -(7i+1)\epsilon}(\cP_{1,D^{(1,i+1)}}) \tensor \TI_{\frac{1}{2} +\gamma - (7i+1)\epsilon }(\cP_{2,D^{(1,i+1)}}))\qstateq] \\
& \ge \Tr[(\TI_{\frac{1}{2}+\gamma -(7i)\epsilon }(\cP_{1,D^{(5,i)}})\tensor \TI_{\frac{1}{2} +\gamma -(7i)\epsilon }(\cP_{2,D^{(5,i)}}))\qstateq] - \delta,
\end{align}
where $\delta$ is some negligible function.
That is, $\Adv_{1}^{i+1} \ge  \Adv_{5}^{i}  - \negl(\secp)$ holds.

\item[$\hybij{4}{q+1}$:] This is the same as $\hybij{3}{q+1}$ except that we change the distribution $D^{(3,q+1)}$ over pairs $(\coin,\ct)$ into $D^{(4,q+1)}$ as follows.
\begin{itemize}
 \item Sample a uniform $\coin \chosen \bit$.
 \item Sample $r^\prime_{\gtag^\ast} \chosen \cR_{\Enc}$ and compute $\ct_{\gtag^\ast} \la \oneSDFE.\Enc(\pk_{\gtag^\ast},x_\coin ;r^\prime_{\gtag^\ast})$, $\prfkey^\prime \la \prfgen^\prime(1^\secp)$, $\prf^\prime_{\ne \gtag^\ast} \la \Puncture^\prime(\prfkey^\prime,\gtag^\ast)$, and $\cthat \gets \iO_2(\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\allowbreak\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}])$ where $\sfE^{\ast\ast}_\sfonefe$ is described in~\cref{fig:enc-one-sdfe-punc-last}. Set $\ct \seteq \cthat$.
 \end{itemize} 


\protocol
{Encryption Circuit $\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast}, x_1,\ct_{\gtag^\ast}](\gtag)$}
{Circuit $\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}]$.
}
{fig:enc-one-sdfe-punc-last}
{
\ifnum\llncs=1
\scriptsize
\else
\fi
\begin{description}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item[Hardwired:] tag $\gtag^\ast$, public key $\pkhat$ (this is an obfuscated circuit), puncturable PRF key $\prf^\prime_{\ne \gtag^\ast}$, plaintext $x_1$, and ciphertext $\ct_{\gtag^\ast}$.
\item[Input:] tag $\gtag \in \zo{\ell}$.
\item[Padding:] circuit is padded to size $\padsize_{\sfE}\seteq\padsize_{\sfE}(\secp,n,s)$, which is determined in analysis.
\end{description}
\begin{enumerate}
\setlength{\parskip}{0.3mm} % between paragraph
\setlength{\itemsep}{0.3mm} % between items
\item If $\gtag^\ast = \gtag$, output $\ct_{\gtag^\ast}$.
\item Else, compute $r^\prime_{\gtag} \gets \prf^\prime_{\ne \gtag^\ast}(\gtag)$ and the circuit $\pkhat$ on input $\gtag$, that is, $\pk_{\gtag} \gets \pkhat(\gtag)$,
\item Output $\ct_{\gtag} \gets \oneSDFE.\Enc(\pk_{\gtag},x_1;r^\prime_{\gtag})$.
\end{enumerate}
}

From the definitions of $\sfE^\ast_{\sfonefe}$, $\sfE^{\ast\ast}_{\sfonefe}$, and $\hybij{3}{q+1}$, the behaviors of $\sfE^{\ast}_{\sfonefe}$ in $\hybij{3}{q+1}$ is the same as that of $\sfE^{\ast\ast}_{\sfonefe}$ in $\hybij{4}{q+1}$.
Moreover, both circuits have the same size by padding $\pad_\sfE$. Then, we can use the indistinguishability of $\iO_2$, and it holds that $D^{(4,q+1)}$ is computationally indistinguishable from $D^{(3,q+1)}$.
This change is for erasing information about $\coin$ from $\sfE^{\ast}_{\sfonefe}$.

By~\cref{thm:ind_distribution_TI}, it holds that
\begin{align}
& \Tr[(\TI_{\frac{1}{2}+\gamma -(7q+5)\epsilon}(\cP_{1,D^{(4,q+1)}}) \tensor \TI_{\frac{1}{2} +\gamma - (7q+5)\epsilon }(\cP_{2,D^{(4,q+1)}}))\qstateq] \\
& \ge \Tr[(\TI_{\frac{1}{2}+\gamma -(7q+4)\epsilon }(\cP_{1,D^{(3,q+1)}})\tensor \TI_{\frac{1}{2} +\gamma -(7q+4)\epsilon }(\cP_{2,D^{(3,q+1)}}))\qstateq] - \delta,
\end{align}
where $\delta$ is some negligible function.
That is, it holds that $\Adv_{4}^{q+1} \ge  \Adv_{3}^{q+1} - \negl(\secp)$.

\item[$\hybi{6}$:] This is the same as $\hybij{4}{q+1}$ except that we choose PRF keys $\prfkey_1,\prfkey_2 \chosen \zo{\secp}$ at the beginning of the game and change the distribution $D^{(4,q+1)}$ over pairs $(\coin,\ct)$ into $D^{(6)}$ as follows.
\begin{itemize}
 \item Sample a uniform $\coin \chosen \bit$.
 \item Sample $r^\prime_{\gtag^\ast} \chosen \cR_{\Enc}$, compute $\ct_{\gtag^\ast} \seteq \oneSDFE.\Enc(\pk_{\gtag^\ast},x_\coin ;r^\prime_{\gtag^\ast})$, $r_1\gets \prf^{(1)}_{\prfkey_1}(\ct_{\gtag^\ast})$, $r_2\gets \prf^{(2)}_{\prfkey_2}(\ct_{\gtag^\ast})$, $\prfkey^\prime \la \PRF^\prime.\Gen(1^\secp;r_1)$, $\prf^\prime_{\ne \gtag^\ast} \la \Puncture^\prime(\prfkey^\prime,\gtag^\ast)$, and $\cthat \seteq \iO_2(\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\allowbreak \prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}];r_2)$ where $\sfE^{\ast\ast}_\sfonefe$ is described in~\cref{fig:enc-one-sdfe-punc-last}. Set $\ct \seteq \cthat$.
 \end{itemize} 
 That is, we de-randomize generation of $\prfkey^\prime$ and $\cthat$. Note that the puncturing algorithm $\Puncture^\prime$ is deterministic in the GGM construction based puncturable PRF~\cite{JACM:GolGolMic86,AC:BonWat13,CCS:KPTZ13,PKC:BoyGolIva14}.
By the pseudorandomness of $\prf^{(1)}$ and $\prf^{(2)}$, $D^{(6)}$ is computationally indistinguishable from $D^{(4,q+1)}$.

By~\cref{thm:ind_distribution_TI}, it holds that
\begin{align}
& \Tr[(\TI_{\frac{1}{2}+\gamma -(7q+7)\epsilon}(\cP_{1,D^{(6)}}) \tensor \TI_{\frac{1}{2} +\gamma - (7q+7)\epsilon }(\cP_{2,D^{(6)}}))\qstateq] \\
& \ge \Tr[(\TI_{\frac{1}{2}+\gamma -(7q+5)\epsilon }(\cP_{1,D^{(4,q+1)}})\tensor \TI_{\frac{1}{2} +\gamma -(7q+5)\epsilon }(\cP_{2,D^{(4,q+1)}}))\qstateq] - 2\delta,
\end{align}
where $\delta$ is some negligible function.
That is, it holds that $\Adv_{6} \ge  \Adv_{4}^{q+1} - \negl(\secp)$.
Note that we use~\cref{thm:ind_distribution_TI} two times here since we use both $\prf^{(1)}$ and $\prf^{(2)}$.
\end{description}

We prove the following.
\begin{lemma}\label{lem:1SDFE_reduction}
If $\oneSDFE$ is challenge-only strong $\gamma/2$-anti-piracy secure, it holds that $\Adv_{6} \le \negl(\secp)$.
\end{lemma}
\begin{proof}[Proof of~\cref{lem:1SDFE_reduction}]
Suppose that $\Adv_{6}$ is non-negligible for a contradiction.
We construct a QPT algorithm $\qB$ for the strong $\gamma/2$-anti-piracy game of $\oneSDFE$ by using the adversary $\qA$ of the strong $\gamma$-anti-piracy game of $\SDFE$ as follows.
\begin{enumerate}
\item  $\qB$ chooses $\gtag_1,\ldots,\gtag_q \chosen \zo{\ell}$ and $\prfkey_1,\prfkey_2 \chosen \zo{\secp}$, and generates $\prfkey \gets \prfgen(1^\secp)$.
\item $\qB$ generates $\prf_{\ne \gtag^\ast} \la \Puncture(\prfkey,\gtag^\ast)$. % and $\prfkey^\prime_{\ne \gtag^\ast} \la \Puncture^\prime(\prfkey^\prime,\gtag^\ast)$.
\item $\qB$ receives $\pk^\ast$ from its challenger, sets $\pk_{\gtag^\ast} \seteq \pk^\ast$, and constructs $\sfS^*_\sfonefe[\gtag^\ast,\prf_{\ne \gtag^\ast},\allowbreak\pk_{\gtag^\ast}]$ described in~\cref{fig:setup-sdfe-punc} by choosing $\gtag^\ast$ for the challenge query $f^\ast$.
$\qB$ sets $\pkhat \seteq \iO_1(\sfS^*_\sfonefe[\gtag^\ast,\prf_{\ne \gtag^\ast},\pk_{\gtag^\ast}])$ and sends it to $\qA$.
\item When $\qA$ sends a key query $f_i$, $\qB$ generates $(\pk_{\gtag_i},\msk_{\gtag_i})\gets \oneSDFE.\Setup(1^\secp;\allowbreak\PRF_{\prfkey_{\ne \gtag^\ast}}(\gtag_i))$ and $\qsk_{f_i,\gtag_i} \gets \oneSDFE.\QKeyGen(\msk_{\gtag_i},f_i)$, sets $\qskhat_{f_i,\gtag_i} \seteq (\gtag_i,\qsk_{f_i,\gtag_i})$, and sends $\qskhat_{f_i}$ to $\qA$.
\item When $\qA$ sends the challenge query $f^\ast$, $\qB$ passes it to its challenger and receives $\qsk_{f^\ast} \gets \oneSDFE.\QKeyGen(\msk^\ast,f^\ast)$, and sends $\qskhat_{f^\ast} \seteq (\gtag^\ast,\qsk_{f^\ast})$ to $\qA$.
\item Again, $\qB$ can answer key queries $f_i$ from $\qA$ as the fourth item.
\item At some point, $\qB$ receives $(x_0,x_1)$ and two (possibly entangled) quantum decryptors $\pirateD_1 = (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2 = (\qstateq[\qreg{R}_2],\mat{U}_2)$, where $f^*(x_0)\ne f^*(x_1)$, from $\qA$. For $i\in \setbk{1,2}$, let $\cP_{i,D^{(6)}}$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
\begin{itemize}
 \item Sample a uniform $\coin \chosen \bit$.
 \item Sample $r^\prime_{\gtag^\ast} \chosen \cR_{\Enc}$, $\ct_{\gtag^\ast} \la \oneSDFE.\Enc(\pk_{\gtag^\ast},x_\coin ;r^\prime_{\gtag^\ast})$.
\item Generate $r_1\gets \prf^{(1)}_{\prfkey_1}(\ct_{\gtag^\ast})$, $r_2\gets \prf^{(2)}_{\prfkey_2}(\ct_{\gtag^\ast})$, $\prfkey^\prime \gets \prfgen^\prime(1^\secp;r_1)$, and $\prf^\prime_{\ne \gtag^\ast}=\Puncture^\prime(\prfkey^\prime,\gtag^\ast)$.
\item Generate $\cthat \gets \iO_2(\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}];r_2)$ where $\sfE^{\ast\ast}_\sfonefe$ is described in~\cref{fig:enc-one-sdfe-punc-last}.
 \item Run the quantum decryptor $(\qstateq^\prime,\mat{U}_i)$ on input $\cthat$. If the outcome is % $f^\ast(x_\coin)$,
 $\coin$, output $1$. Otherwise, output $0$.
\end{itemize}
\item $\qB$ sets quantum decryptors $\pirateD_1^\ast$ and $\pirateD_2^\ast$ as follows.

In this item, we denote pure state $\ket{x}\bra{x}$ by $\ket{x}$ for ease of notation.
First, $\qB$ constructs $(\qstateq^\ast[\qreg{R}_i],\mat{U}_i^\ast)$ such that
\begin{itemize}
\item Set  $\qstateq^\ast[\qreg{R}_i] \seteq \qstateq[\qreg{R}_i] \tensor \ket{0^{\abs{\cthat}}} \tensor \ket{\gtag^\ast, \pkhat, 0^\ell, x_1, \prfkey_1,\prfkey_2,0^{\abs{r_1}},0^{\abs{r_2}},0^{\ell}} \tensor \ket{\ct_{\gtag^\ast}}$. Note that $\ket{\ct_{\gtag^\ast}}$ is the input for $(\qstateq^\ast[\qreg{R}_i],\mat{U}_i^\ast)$.
\item Unitary $\mat{U}^\ast_i$ acts on $\qstateq^\ast[\qreg{R}_i]$ and the result is
\[
\qstateq^\prime[\qreg{R}_i] \seteq \qstateq[\qreg{R}_i] \tensor \ket{\cthat} \tensor \ket{\gtag^\ast, \pkhat, \prf^\prime_{\ne \gtag^\ast}, x_1,\prfkey_1,\prfkey_2,r_1,r_2,\prfkey^\prime}\tensor \ket{\ct_{\gtag^\ast}},
\]
where $r_1 \seteq \prf^{(1)}_{\prfkey_1}(\ct_{\gtag^\ast})$, $r_2 \seteq \prf^{(2)}_{\prfkey_2}(\ct_{\gtag^\ast})$, $\prfkey^\prime \seteq \prfgen^\prime(1^\secp;r_1)$, $\prf^\prime_{\ne \gtag^\ast} \seteq \Puncture^\prime(\prfkey^\prime,\gtag^\ast)$, and $\cthat \seteq  \iO_2(\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}];r_2)$. That is, $\mat{U}_i^\ast$ constructs $\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}]$ described in~\cref{fig:enc-one-sdfe-punc-last} and generates $\cthat \seteq \iO_2(\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}];r_2)$. Note that $\qB$ can construct it since $\qB$ has $\gtag^\ast$, $\pkhat$, $\prfkey_1$, $\prfkey_2$, and $x_1$.
\end{itemize}
It is easy to see that if we apply $(\mat{U}_i \tensor \mat{I})$ to $\qstateq^\prime[\qreg{R}_i]$, we obtain an output of $\pirateD_i$ for input $\cthat$.
Thus, $\qB$ sets $\pirateD_1^\ast \seteq (\qstateq^\ast[\qreg{R}_1],(\mat{U}_1\tensor \mat{I})\mat{U}_1^\ast)$ and $\pirateD_2^\ast \seteq (\qstateq^\ast[\qreg{R}_2],(\mat{U}_2 \tensor \mat{I})\mat{U}_2^\ast)$.
$\qB$ sends $(x_0,x_1)$ and $\pirateD_1^\ast$ and $\pirateD_2^\ast$ to its challenger.
\end{enumerate}
The challenger of $\oneSDFE$ runs the test by using the following.
Let $\cP_{i,D^\prime}$ be the following mixture of projective measurements acting on some quantum state $\qstateq_{\oneSDFE}$:
\begin{itemize}
\item Sample a uniformly random $\coin\chosen \bit$ and compute $\ct_{\gtag^\ast} \gets \oneSDFE.\Enc(\pk_{\gtag^\ast},\allowbreak x_\coin)$.
\item Run $\coin^\prime \gets \pirateD^\ast(\ct)$. If $\coin^\prime = \coin$, output $1$, otherwise output $0$.
\end{itemize}

By the construction of $\mat{U}_i^\ast$, quantum decryptor $\pirateD_i^\ast$ takes a ciphertext $\ct_{\gtag^\ast}$ under $\pk_{\gtag^\ast}$ as input, converts it into a ciphertext $\cthat$ of $\SDFE$, and apply the quantum decryptor $\pirateD_i$ from $\qA$. The converted ciphertext $\cthat$ perfectly simulates a ciphertext in $\hybi{6}$ if an input to $\pirateD_i^\ast$ is a ciphertext under $\pk_{\gtag^\ast}$.


We assumed that $\Adv_{6}$ is non-negligible at the beginning of this proof.
That is, applying $\TI_{\frac{1}{2}+\gamma -(7q+7)\epsilon}(\cP_{i,D^{(6)}})$ on $\qstateq^\ast[\qreg{R}_i]$ results in two outcomes $1$ with non-negligible probability.
That is, it holds that
\begin{align}
\Tr[\TI_{\frac{1}{2}+\gamma -(7q+7)\epsilon}(\cP_{1,D^{(6)}}) \tensor \TI_{\frac{1}{2}+\gamma - (7q+7)\epsilon}(\cP_{2,D^{(6)}})\qstateq^\ast] > \negl(\secp).
\end{align}
This means that for $i\in \setbk{1,2}$, $\qstateq^\ast[\qreg{R}_i]$ is a $(\gamma -(7q+7)\epsilon)$-good distinguisher with respect to ciphertexts generated according to $D^{(6)}$.


Thus, if $\pirateD_i$ works as a $(\gamma- (7q+7)\epsilon)$-good quantum distinguisher for $\SDFE$, $\pirateD_i^\ast$ works as a $(\gamma - (7q+7) \epsilon )$-good quantum distinguisher for $\oneSDFE$, where $\epsilon= \frac{\gamma}{2(7q+7)}$. This completes the proof of~\cref{lem:1SDFE_reduction}.
\end{proof}

By using the relationships among $\adva{\SDFE,\qA}{}$, $\Adv_{x}^{i}$ for $x\in \setbk{1,\cdots,5}$ and $i\in [q]$, $\Adv_{x}^{q+1}$ for $x\in \setbk{1,\cdots,4}$, and $\Adv_6$ that we show above, we obtain $\advc{\SDFE,\qA}{strong}{anti}{piracy}(\secp,\gamma) \le \negl(\secp)$.
We almost complete the proof of~\cref{thm:SDFE_anti-piracy_from_1SDFE_IO}. Lastly, we need to set the padding parameters for IO security.

\paragraph{Padding Parameter.} The proof of security relies on the indistinguishability of obfuscated $\sfS_{\sfonefe}$ and $\sfS^*_{\sfonefe}$ defined in Figures~\ref{fig:setup-pkfe} and \ref{fig:setup-sdfe-punc},
and that of obfuscated $\sfE_\sfonefe$, $\sfE_\sfonefe^\ast$, and $\sfE_\sfonefe^{\ast\ast}$ defined in~\cref{fig:enc-one-pkfe,fig:enc-one-sdfe-punc,fig:enc-one-sdfe-punc-last}. Accordingly, we set $\padsize_{\sfS} \seteq \max(\abs{\sfS_{\sfonefe}},\abs{\sfS_{\sfonefe}^*})$ and $\padsize_{\sfE} \seteq \max(\abs{\sfE_{\sfonefe}},\abs{\sfE_{\sfonefe}^*},\abs{\sfE_\sfonefe^{\ast\ast}})$.

The circuits $\sfS_\sfonefe$ and $\sfS_\sfonefe^*$ compute a puncturable PRF over domain $\zo{\ell}$ and a key pair of $\oneFE$, and may have punctured PRF keys and a public key hardwired. The circuits $\sfE_\sfonefe$, $\sfE_\sfonefe^*$, and $\sfE_\sfonefe^{\ast\ast}$ run the circuit $\pkhat$ and compute a puncturable PRF over domain $\zo{\ell}$ and a ciphertext of $\oneSDFE$, and may have punctured PRF keys, tags, plaintexts, and a hard-wired ciphertext. Note that $\ell$ is a polynomial of $\secp$. Thus, it holds that
 \begin{align}
 \pad_{\sfS} & \le \poly(\secp,n,s),\\
 \pad_{\sfE} & \le \poly(\secp,n,s,\abs{\pkhat}).
 \end{align}
 Therefore, we complete the proof of~\cref{thm:SDFE_anti-piracy_from_1SDFE_IO}.
\end{proof}

We obtain the following corollary from~\cref{cor:strong_1SDFE_from_IO_LWE,thm:SDFE_from_1FE_IO,thm:SDFE_anti-piracy_from_1SDFE_IO}.

\begin{corollary}\label{cor:strong_SDFE_from_IO_LWE}
Assuming the existence of sub-exponentially secure IO for $\Ppoly$, and the hardness of QLWE, there exists an SDFE scheme for $\Ppoly$ that satisfies adaptive security (\cref{def:adaptive_SDFE}) and strong $\gamma$-anti-piracy security for any inverse polynomial $\gamma$.
\end{corollary}




%%%%%% OLD proof for single-key strong anti-piracry %%%%%%
% \begin{proof}
% We define a sequence of hybrid games to prove the theorem.
% \begin{description}
% \item[$\hybi{0}$:] This is the same as $\expc{\qA,\oneSDFE}{strong}{anti}{piracy}(\secp,\gamma(\secp))$. The detailed description is as follows.
% \begin{enumerate}
% \item Compute $(\fe.\pk,\fe.\msk) \gets \PKFE.\Setup(1^\secp)$ and $(\sde.\pk,\sde.\dk)\gets\SDE.\Setup(1^\secp)$. Set $\pk \seteq (\fe.\pk,\sde.\pk)$ and $\msk \seteq (\fe.\msk,\sde.\dk)$.
% \item Compute $\fe.\sk_{f^\ast} \gets \PKFE.\KG(\fe.\msk,f^\ast)$ and $\sde.\qdk \gets \SDE.\QKeyGen(\sde.\dk)$, and  send $\qsk_{f^\ast} \seteq (\fe.\sk_{f^\ast},\sde.\qdk)$ to $\qA$.
% \item Receive $(x_0,x_1)$, $\pirateD_1 =(\qstateq[\qreg{R}_1],\mat{U}_1)$, and $\pirateD_2 =(\qstateq[\qreg{R}_2],\mat{U}_2)$, where $f^\ast(x_0)\ne f^\ast(x_1)$.
% \item For $i\in \setbk{1,2}$, let $\cP_{i,D}$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
% \begin{itemize}
% \item Sample a uniform $\coin \chosen \bit$. Compute $\fe.\ct \gets \PKFE.\Enc(\fe.\pk,x_\coin)$ and $\sde.\ct \gets \SDE.\Enc(\sde.\pk,\fe.\ct)$ and set $\ct \seteq \sde.\ct$.
% \item Run the quantum decryptor $(\qstateq^\prime,\mat{U}_i)$ on input $\ct$. If the outcome is % $f^\ast(x_\coin)$,
% $\coin$, output $1$. Otherwise, output $0$.
% \end{itemize}
% Let $D$ be the distribution over pairs $(\coin,\ct)$ defined in the first item above, and let $\cE_i = \setbk{\mat{E}^i_{(\coin,\ct)}}_{\coin,\ct}$ be a collection of projective measurements where $\mat{E}^i_{(\coin,\ct)}$ is the projective measurement described in the second item above.
% $\cP_{i,D}$ is the mixture of projective measurements associated to $D$ and $\cE_i$.
% \item Run $\TI_{\frac{1}{2}+\gamma}(\cP_{i,D})$ for $i\in \setbk{1,2}$ on quantum decryptor $\pirateD_1=(\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2=(\qstateq[\qreg{R}_2],\mat{U}_2)$.
% Output $1$ if both tests pass, otherwise output $0$.
% \end{enumerate}


% \item[$\hybi{1}$:] This is the same as $\hybi{0}$ except that the challenger runs $\ATI^{\epsilon,\delta}_{\cE_1,D,\frac{1}{2}+\gamma-\epsilon}$ and $\ATI^{\epsilon,\delta}_{\cE_2,D,\frac{1}{2}+\gamma-\epsilon}$, where $\epsilon=\frac{\gamma}{4}$, and $\delta$ is some negligible function of $\secp$, instead of $\TI_{\frac{1}{2}+\gamma}(\cP_{i,D})$.
% \end{description}
% Let $\adva{\SDFE,\qA}{1}$ be the advantage of $\qA$ in $\hybi{1}$.
% It holds that
% \begin{align}
% \advc{\SDFE,\qA}{strong}{anti}{piracy}(\secp,\gamma(\secp)) - \adva{\SDFE,\qA}{1}\le 2\delta \label{eq:1SDFE_ATI}
% \end{align}

% by~\cref{lem:ATI_bipartite_app}.
% For $i\in\setbk{1,2}$, $\ATI^{\epsilon,\delta}_{\cE_i,D,\frac{1}{2}+\gamma-\epsilon}$ runs in time $\poly(\log{(1/\delta)},1/\epsilon)$ by~\cref{lem:ATI_property}. Since we set $\epsilon = \gamma/4$, $\poly(\log{(1/\delta)},1/\epsilon)$ is polynomial.

% We prove the following.
% \begin{lemma}\label{lem:1SDFE_hyb1}
% If $\SDE$ is strong $\gamma/4$-anti-piracy secure for randomized message, it holds that $\adva{\SDFE,\qA}{1} \le \negl(\secp)$.
% \end{lemma}
% \begin{proof}[Proof of~\cref{lem:1SDFE_hyb1}]
% Suppose that $\adva{\SDFE,\qA}{1}$ is non-negligible for a contradiction.
% We construct a QPT algorithm $\qB$ for the strong $\gamma$-anti-piracy game with randomized function $\setbk{\PKFE.\Enc(\fe.\pk,\cdot;\cdot)}_{\secp}$ of $\SDE$ by using the adversary $\qA$ of the strong $\gamma$-anti-piracy game of $\SDFE$ as follows.
% \begin{enumerate}
% \item $\qB$ receives $\sde.\pk$ and $\sde.\qdk$ from its challenger.
% \item $\qB$ generates $(\fe.\pk,\fe.\msk) \gets \PKFE.\Setup(1^\secp)$, sets $\pk\seteq (\fe.\pk,\sde.\pk)$, and sends it to $\qA$.
% \item When $\qA$ sends the challenge query $f^\ast$, $\qB$ generates $\fe.\sk_{f^\ast} \gets \PKFE.\KG(\fe.\msk,f^\ast)$, sets $\qsk_{f^\ast} \seteq (\fe.\sk_{f^\ast},\sde.\qdk)$, and sends $\qsk_{f^\ast}$ to $\qA$.
% \item At some point, $\qB$ receives $(x_0,x_1)$ and two (possibly entangled) quantum decryptors $\pirateD_1 = (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2 = (\qstateq[\qreg{R}_2],\mat{U}_2)$, where $f^*(x_0)\ne f^*(x_1)$, from $\qA$. For $i\in \setbk{1,2}$, let $\cP_{i,D}$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
% \begin{itemize}
% \item Sample a uniform $\coin \chosen \bit$. Compute $\fe.\ct \gets \PKFE.\Enc(\fe.\pk,x_\coin)$ and $\sde.\ct \gets \SDE.\Enc(\sde.\pk,\fe.\ct)$ and set $\ct \seteq \sde.\ct$.
% \item Run the quantum decryptor $(\qstateq^\prime,\mat{U}_i)$ on input $\ct$. If the outcome is % $f^\ast(x_\coin)$,
% $\coin$, output $1$. Otherwise, output $0$.
% \end{itemize}
% $\qB$ runs $\ATI^{\epsilon,\delta}_{\cE_1,D,\frac{1}{2}+\gamma-\epsilon}$ and $\ATI^{\epsilon,\delta}_{\cE_2,D,\frac{1}{2}+\gamma-\epsilon}$ on quantum decryptor $\pirateD_1=(\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2=(\qstateq[\qreg{R}_2],\mat{U}_2)$.
% $\qB$ aborts if either of the tests does not pass, otherwise proceeds to the next step.
% Let $\qstateq^\ast$ be the bipartite state conditioned on both outcomes being $1$.
% \item $\qB$ sets quantum decryptors $\pirateD_1^\ast$ and $\pirateD_2^\ast$ as follows.
% $\qB$ sets $\pirateD_1^\ast \seteq (\qstateq^\ast[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2^\ast \seteq (\qstateq^\ast[\qreg{R}_2],\mat{U}_2)$.
% $\qB$ sets an injective randomized function $g(\cdot;\cdot)\seteq \PKFE.\Enc(\fe.\pk,\cdot;\cdot)$ and sends $(x_0,x_1,g))$ and $\pirateD_1^\ast = (\qstateq^\ast[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2^\ast = (\qstateq^\ast[\qreg{R}_2],\mat{U}_2)$ to its challenger.
% \end{enumerate}
% By the condition $f^\ast(x_0) \ne f^\ast(x_1)$, it holds that $x_0 \ne x_1$.
% By the perfect correctness of $\PKFE$, $\PKFE.\Enc(\fe.\pk,\cdot;\cdot)$ is an injective randomized function.\footnote{If $\Enc(\fe.\pk,x_0;r_0)= \Enc(\fe.\pk,x_1;r_1)$ holds, we obtain $f^\ast(x_0)=\Dec(\fe.\sk_{f^\ast},\Enc(\fe.\pk,x_0;r_0)) = \Dec(\fe.\sk_{f^\ast},\Enc(\fe.\pk,x_1;r_1))=f^\ast(x_1)$. This contradicts to $f^\ast(x_0)\ne f^\ast(x_1)$.} The challenger of $\SDE$ runs the test by using the following.
% Let $\cP_{i,D^\prime}$ be the following mixture of projective measurements acting on some quantum state $\qstateq_{\SDE}$:
% \begin{itemize}
% \item Sample a uniformly random $\coin\chosen \bit$ and $r \chosen \cR$, and compute $m_\coin^\prime \seteq \PKFE.\Enc(\fe.\pk,x_\coin;r)$. Note that $\qB$ sets $g(\cdot,\cdot) \seteq \PKFE.\Enc(\fe.\pk,\cdot;\cdot)$. Then, compute $\ct \gets \SDE.\Enc(\sde.\pk,m_\coin^\prime)$.
% \item Run $\coin^\prime \gets \pirateD(\ct)$. If $\coin^\prime = \coin$, output $1$, otherwise output $0$.
% \end{itemize}
% The distribution is the same as $D$, which $\qB$ simulates.

% We assumed that $\adva{\SDFE,\qA}{1}$ is non-negligible at the begging of this proof.
% That is, applying $\ATI^{\epsilon,\delta}_{\cE_i,D,\frac{1}{2}+\gamma-\epsilon}$ on $\qstateq^\ast[\qreg{R}_i]$ results in two outcomes $1$ with non-negligible probability.
% By the second item of~\cref{lem:ATI_bipartite_app}, it holds that
% \begin{align}
% \Tr[\TI_{\frac{1}{2}+\gamma - 3\epsilon}(\cP_{1,D}) \tensor \TI_{\frac{1}{2}+\gamma - 3\epsilon}(\cP_{2,D})\qstateq^\ast] \ge 1- 4\delta.
% \end{align}
% This means that $\qstateq^\ast[\qreg{R}_i]$ is negligibly close to being a $(\gamma -3\epsilon)$-good decryptor with respect to ciphertexts generated according to $D$. Recall that $\delta$ is some negligible function.
% It is easy to see that $(\pirateD_1^\ast,\pirateD_2^\ast)$ is a $(\gamma-3\epsilon)$-good decryptor for randomized function $\PKFE.\Enc(\fe.\pk,\cdot;\cdot)$.
% Thus, if $\qA$ outputs $\gamma$-good decryptor, $\qB$ can also outputs $(\gamma-3\epsilon)$-good decryptor for randomized function $\PKFE.\Enc(\fe.\pk,\cdot;\cdot)$. Recall that we set $\epsilon= \frac{\gamma}{4}$. This completes the proof of~\cref{lem:1SDFE_hyb1}.
% \end{proof}
% By~\cref{eq:1SDFE_ATI,lem:1SDFE_hyb1}, we complete the proof of~\cref{thm:1SDFE_anti-piracy_from_SDE}.
% \end{proof}





%%%%%% OLD proof for collusion-resistant strong anti-piracry %%%%%
% \begin{proof}[Proof of~\cref{thm:SDFE_anti-piracy_from_1SDFE_IO}]
% Let $\qA$ be an adversary attacking the strong $\gamma$-anti-piracy of $\SDFE$.
% We define a sequence of hybrid games.
% For the hybrid games, we define the following values.
% Let $q$ be the total number of key queries by $\qA$ except the challenge query $f^\ast$. Note that $q$ could be any polynomial.
% When we start the strong $\gamma$-anti-piracy security game, the adversary $\qA$ is fixed and $q$ is also fixed. We choose tags $\gtag_1,\ldots,\gtag_q \chosen \zo{\ell}$ for $q$ key queries and $\gtag^\ast$ for the challenge query at the beginning of the game.
% We can sort these tags except $\gtag^\ast$ in the ascending order $\gtag_{j_1}<  \cdots < \gtag_{j_{q}}$ where $j_i \in [q]$.
% We can interpret $\ell$ bit strings as integers and assume that there is no $i,j$ such that $i\ne j$ and $\gtag_i = \gtag_j$ without loss of generality.
% We rename $\gtag^\prime_{i} \seteq \gtag_{j_i}$. It trivially holds that $\gtag^\prime_{1}<  \cdots < \gtag^\prime_{q}$.
% Our reduction algorithm can identify which $\gtag^\prime_i$ should be used when it receives the $k$-th query since it can have a permutation $\pi$ such that $\gtag^\prime_{\pi(k)} = \gtag_{k}$.
% We also sets $\gtag^\prime_{q+1}\seteq \gtag^\ast$.

% \begin{description}
% \item[$\hybi{0}$:] The first game is the original strong $\gamma$-anti-piracy experiment, that is, $\expc{\SDFE,\qA}{strong}{anti}{piracy}(1^\secp,\gamma)$.
% \begin{enumerate}
% \item The challenger generates $(\pkhat,\mskhat)=(\iO_1(\sfS_\sfonefe),\prfkey)\gets \SDFE.\Setup(1^\secp)$ and sends $\pkhat$ to $\qA$.
% \item $\qA$ sends key queries $f_k$ to the challenger and the challenger returns $\qskhat_{f_k} = (\gtag_k,\qsk_{f_k,\gtag_k}) \lrun \SDFE.\QKeyGen(\mskhat,f_k)$ where $\qsk_{f_k,\gtag_k}\lrun \oneSDFE.\QKeyGen(\msk_{\gtag_k},f_k)$.
% \item At some point $\qA$ sends a challenge query $f^*$ to the challenger and the challenger returns $\qskhat =(\gtag^\ast,\qsk_{f^\ast}) \lrun \SDFE.\QKeyGen(\mskhat,f^\ast)$ where $\qsk_{f^\ast}\lrun \oneSDFE.\QKeyGen(\msk_{\gtag^\ast},f^*)$.
% \item Again, $\qA$ sends $f_k$ to the challenger and the challenger returns $\qskhat_{f_k} \lrun \SDFE.\QKeyGen(\mskhat,f_k)$.
% \item $\qA$ outputs $(x_0,x_1)$ and two (possibly entangled) quantum decryptors $\pirateD_1 = (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2 = (\qstateq[\qreg{R}_2],\mat{U}_2)$, where $\forall i\ f_i(x_0)=f_i(x_1)$, $f^*(x_0)\ne f^*(x_1)$, $\qstateq$ is a quantum state over registers $\qreg{R}_1$ and $\qreg{R}_2$, and $\mat{U}_1$ and $\mat{U}_2$ are general quantum circuits.
% \item For $i\in \setbk{1,2}$, let $\cP_{i,D}$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
% \begin{itemize}
% \item Sample a uniform $\coin \chosen \bit$. Compute $\cthat \gets \SDFE.\Enc(\pkhat,x_\coin)$ and set $\ct \seteq \cthat$.
% \item Run the quantum decryptor $(\qstateq^\prime,\mat{U}_i)$ on input $\ct$. If the outcome is % $f^\ast(x_\coin)$,
% $\coin$, output $1$. Otherwise, output $0$.
% \end{itemize}
% Let $D$ be the distribution over pairs $(\coin,\ct)$ defined in the first item above, and let $\cE_i = \setbk{\mat{E}^i_{(\coin,\ct)}}_{\coin,\ct}$ be a collection of projective measurements where $\mat{E}^i_{(\coin,\ct)}$ is the projective measurement described in the second item above.
% $\cP_{i,D}$ is the mixture of projective measurements associated to $D$ and $\cE_i$.
% \item The challenger runs the test for a $\gamma$-good FE decryptor with respect to $\pk$, $(x_0,x_1)$, and $f^\ast$ on $\pirateD_1$ and $\pirateD_2$.
% The challenger outputs $1$ if both tests pass, otherwise outputs $0$.
% \end{enumerate}
% Let $\Adv_{x}^{i}$ be the advantage of $\qA$ in $\hybij{x}{i}$.

% \item[$\hybij{1}{0}$:] This is the same as $\hybi{1}$\fuyuki{$\hybi{0}$?} except that the challenger run $\ATI^{\epsilon,\delta}_{\cE_1,D,\frac{1}{2}+\gamma-\epsilon}$ and $\ATI^{\epsilon,\delta}_{\cE_2,D,\frac{1}{2}+\gamma -\epsilon}$, where $\epsilon=\frac{\gamma}{2(24q+24)}$, and $\delta$ is some negligible function of $\secp$.
% Note that we can set $\epsilon$ to any inverse polynomial and $\gamma$ is any inverse polynomial.

% It holds that
% $\Adv_{1}^{0}  \ge \advc{\SDFE,\qA}{strong}{anti}{piracy} - 2\delta$ by~\cref{lem:ATI_bipartite_app}.
% For $b\in\setbk{1,2}$, $\ATI^{\epsilon,\delta}_{\cE_b,D,\frac{1}{2}+\gamma-\epsilon}$ runs in time $\poly(\log{(1/\delta)},1/\epsilon)$ by~\cref{lem:ATI_property}. Since we set $\epsilon = \frac{\gamma}{2(24q+24)}$ and $q$ is a polynomial, $\poly(\log{(1/\delta)},1/\epsilon)$ is polynomial.

% \item[$\hybij{1}{i}$:] This is defined for $i \in [q+1]$ and the same as $\hybij{5}{i-1}$ except that we generate $\pkhat$ as obfuscated $\sfS^*_\sfonefe$ described in~\cref{fig:setup-sdfe-punc}. Note that we define $\hybij{5}{0}=\hybij{1}{0}$. In this hybrid game, we set $r_{\gtag^\prime_i} \la \prf_{\prfkey}(\gtag^\prime_i)$, $\prf_{\ne \gtag^\prime_i} \la \Puncture(\prfkey,\gtag^\prime_i)$, and $(\pk_{\gtag^\prime_i},\msk_{\gtag^\prime_i}) \la \oneSDFE.\Setup(1^\secp ;r_{\gtag^\prime_i})$.

% The behavior of $\sfS^*_\sfonefe$ is the same as that of $\sfS_\sfonefe$ since the hard-wired $\pk_{\gtag^\prime_1}$ in $\sfS^*_\sfonefe$ is the same as the output of $\sfS_\sfonefe$ on the input $\gtag^\prime_1$. Their size is also the same since we pad circuit $\sfS_\sfonefe$ to have the same size as $\sfS_\sfonefe^*$. Then, we can use the indistinguishability guarantee of $\iO_1$ and it holds that $\iO_1(\sfS_\sfonefe[\prfkey])$ is computationally indistinguishable from $\iO_1(\sfS^\ast_\sfonefe[\gtag^\prime_i,\prf_{\ne \gtag^\prime_i},\pk_{\gtag^\prime_i}])$. Let $D^{(1,i)}$ be the distribution over pairs $(\coin,\ct)$ defined in $\hybi{0}$ except that $\iO_1(\sfS^\ast_\sfonefe[\gtag^\prime_i,\prf_{\ne \gtag^\prime_i},\pk_{\gtag^\prime_i}])$ as $\pkhat$. Then, $D^{(1,1)}$ is computationally indistinguishable from $D$.

% In this hybrid game, we also use $\ATI^{\epsilon,\delta}_{\cE_b,D^{(1,1)},\frac{1}{2}+\gamma-\epsilon- (24i-21) \epsilon}$ instead of $\ATI^{\epsilon,\delta}_{\cE_b,D,\frac{1}{2}+\gamma-\epsilon}$.
% By~\cref{cor:ind_distribution_ATI}, it holds that
% \begin{align}
% & \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(1,1)},\frac{1}{2}+\gamma -\epsilon -3\epsilon } \tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(1,1)},\frac{1}{2} +\gamma - \epsilon -3\epsilon})\qstateq] \\
% & \ge \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{},\frac{1}{2}+\gamma -\epsilon}\tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{},\frac{1}{2} +\gamma -\epsilon})\qstateq] - 3\delta,
% \end{align}
% where $\delta^\prime$ is some negligible function.
% That is, it holds that $ \Adv_{1}^{1} \ge  \Adv_{1}^{0} - \negl(\secp)$.

% \item[$\hybij{2}{i}$:] This is defined for $i \in [q+1]$ and the same as $\hybij{1}{i}$ except that we change the distribution $D^{(1,i)}$ over pairs $(\coin,\ct)$ into $D^{(2,i)}$ as follows.
% \begin{itemize}
%  \item Sample a uniform $\coin \chosen \bit$.
%  \item Compute $r^\prime_{\gtag^\prime_i} \la \prf^\prime_{\prfkey^\prime}(\gtag^\prime_i)$, $\prf^\prime_{\ne \gtag^\prime_i} \la \Puncture^\prime(\prfkey^\prime,\gtag^\prime_i)$, $\ct_{\gtag^\prime_i} \la \oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_\coin ;r^\prime_{\gtag^\prime_i})$, and $\cthat \gets \iO_2(\sfE^\ast_\sfonefe[\gtag^\prime_i,\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\prime_i},x_\coin,x_1,\ct_{\gtag^\prime_i}])$ where $\sfE^\ast_\sfonefe$ is described in~\cref{fig:enc-one-sdfe-punc}. Set $\ct \seteq \cthat$.
%  \end{itemize} 

% \protocol
% {Setup Circuit $\sfS^*_{\sfonefe} [\gtag^\prime,\prf_{\ne \gtag^\prime},\pk_{\gtag^\prime}](\gtag)$}
% {Circuit $\sfS^*_{\sfonefe} [\gtag^\prime,\prf_{\ne \gtag^\prime},\pk_{\gtag^\prime}]$.
% }
% {fig:setup-sdfe-punc}
% {
% \ifnum\llncs=1
% \scriptsize
% \else
% \fi
% \begin{description}
% \setlength{\parskip}{0.3mm} % between paragraph
% \setlength{\itemsep}{0.3mm} % between items
% \item[Hardwired:] tag $\gtag^\prime$, puncturable PRF key $\prf_{\ne \gtag^\prime}$, and $\oneSDFE$ public-key $\pk_{\gtag^\prime}$.
% \item[Input:] tag $\gtag \in \zo{\ell}$.
% \item[Padding:] circuit is padded to size $\padsize_{\sfS}\seteq\padsize_{\sfS}(\secp,n,s)$, which is determined in analysis.
% \end{description}
% \begin{enumerate}
% \setlength{\parskip}{0.3mm} % between paragraph
% \setlength{\itemsep}{0.3mm} % between items
% \item If $\gtag^\prime = \gtag$, output $\pk_{\gtag^\prime}$.
% \item Else, compute $r \gets \prf_{\ne \gtag^\prime}(\gtag)$.
% \item Compute $(\pk_{\gtag}, \msk_{\gtag}) \gets \oneSDFE.\Setup(1^\secp;r_i)$ and output $\pk_{\gtag}$.
% \end{enumerate}
% }


% \protocol
% {Encryption Circuit $\sfE^*_\sfonefe[\gtag^\prime,\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\prime},x_\coin, x_1,\ct_{\gtag^\prime}](\gtag)$}
% {Circuit $\sfE^*_\sfonefe[\gtag^\prime,\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\prime},x_\coin,x_1,\ct_{\gtag^\prime}]$.
% }
% {fig:enc-one-sdfe-punc}
% {
% \ifnum\llncs=1
% \scriptsize
% \else
% \fi
% \begin{description}
% \setlength{\parskip}{0.3mm} % between paragraph
% \setlength{\itemsep}{0.3mm} % between items
% \item[Hardwired:] tags $\gtag^\prime$, $\gtag^\ast$, public key $\pkhat$ (this is an obfuscated circuit), puncturable PRF key $\prf^\prime_{\ne \gtag^\prime}$, plaintexts $x_\coin,x_1$, and ciphertext $\ct_{\gtag^\prime}$.
% \item[Input:] tag $\gtag \in \zo{\ell}$.
% \item[Padding:] circuit is padded to size $\padsize_{\sfE}\seteq\padsize_{\sfE}(\secp,n,s)$, which is determined in analysis.
% \end{description}
% \begin{enumerate}
% \setlength{\parskip}{0.3mm} % between paragraph
% \setlength{\itemsep}{0.3mm} % between items
% \item If $\gtag^\prime = \gtag$, output $\ct_{\gtag^\prime}$.
% \item Else, compute $r^\prime_{\gtag} \gets \prf^\prime_{\ne \gtag^\prime_i}(\gtag)$ and the circuit $\pkhat$ on input $\gtag$, that is, $\pk_{\gtag} \gets \pkhat(\gtag)$,
% \begin{description}
%     \item[If $\gtag = \gtag^\ast$:] Output $\ct_{\gtag^\ast} \gets \oneSDFE.\Enc(\pk_{\gtag^\ast},x_\coin;r^\prime_{\gtag^\ast})$
% \item[If $\gtag > \gtag^\prime$:] Output $\ct_\gtag \gets \oneSDFE.\Enc(\pk_{\gtag},x_\coin;r^\prime_{\gtag})$.
% \item[If $\gtag < \gtag^\prime$:] Output $\ct_\gtag \gets \oneSDFE.\Enc(\pk_{\gtag},x_1;r^\prime_{\gtag})$.
% \end{description}
% \end{enumerate}
% }


% The behavior of $\sfE^*_\sfonefe$ is the same as that of $\sfE_\sfonefe$ since the hard-wired $\ct_{\gtag^\prime_i}$ in $\sfE^*_\sfonefe$ is the same as the output of $\sfE_\sfonefe$ on the input $\gtag^\prime_i$.
% Moreover, both circuits have the same size by padding $\pad_\sfE$. Then, we can use the indistinguishability guarantee of $\iO_2$ and it holds that $D^{(2,i)}$ is computationally indistinguishable from $D^{(1,i)}$.

% In this hybrid game, we also use $\ATI^{\epsilon,\delta}_{\cE_1,D^{(2,i)},\frac{1}{2}+\gamma -\epsilon -(24i-18)\epsilon}$ instead of $\ATI^{\epsilon,\delta}_{\cE_2,D^{(1,i)},\frac{1}{2}+\gamma-(24i-21)\epsilon}$.

% By~\cref{cor:ind_distribution_ATI}, it holds that
% \begin{align}
% & \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(2,i)},\frac{1}{2}+\gamma -\epsilon -(24i-18)\epsilon}  \tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(2,i)},\frac{1}{2} +\gamma -\epsilon -(24i - 18)\epsilon})\qstateq]  \\
% &\ge \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(1,i)},\frac{1}{2}+\gamma -\epsilon -(24i-21)\epsilon}\tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(1,i)},\frac{1}{2} +\gamma -\epsilon -(24i- 21)\epsilon})\qstateq] - 3\delta.
% \end{align}
% That is, it holds that $\Adv_{2}^{i} \ge  \Adv_{1}^{i}  -\negl(\secp)$.

% \item[$\hybij{3}{i}$:] This is defined for $i \in [q+1]$ and the same as $\hybij{2}{i}$ except that we use distribution $D^{(3,i)}$, which is the same as $D^{(2,i)}$ except that setup randomness $r_{\gtag^\ast}\chosen \cR_{\Setup}$ and encryption randomness $r^\prime_{\gtag^\ast}\chosen \cR_{\Enc}$ are uniformly random. By the punctured pseudorandomness of $\prf$ and $\prf^\prime$, $D^{(3,i)}$ is computationally indistinguishable from $D^{(2,i)}$.

% In this hybrid game, we also use $\ATI^{\epsilon,\delta}_{\cE_b,D^{(3,i)},\frac{1}{2}+\gamma-\epsilon- (24i-12) \epsilon}$ instead of $\ATI^{\epsilon,\delta}_{\cE_b,D^{(2,i)},\frac{1}{2}+\gamma-(24i-18)\epsilon}$.

% By~\cref{cor:ind_distribution_ATI}, it holds that
% \begin{align}
% & \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(3,i)},\frac{1}{2}+\gamma -\epsilon -(24i-12)\epsilon} \tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(3,i)},\frac{1}{2} +\gamma -\epsilon -(24i-12)\epsilon})\qstateq] \\
% & \ge \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(2,i)},\frac{1}{2}+\gamma -\epsilon -(24i-18)\epsilon}\tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(2,i)},\frac{1}{2} +\gamma-\epsilon -(24i-18)\epsilon})\qstateq] - 3\delta.
% \end{align}
% That is, it holds that $\Adv_{3}^{i} \ge  \Adv_{2}^{i} - \negl(\secp)$.
% Note that we apply \cref{thm:ind_distribution_TI} twice here since we use punctured pseudorandomness of both $\prf$ and $\prf^\prime$.

% \item[$\hybij{4}{i}$:] This is defined for $i \in [q]$ and the same as $\hybij{3}{i}$ except that we use distribution $D^{(4,i)}$, which is the same as $D^{(3,i)}$ except that the ciphertext $\ct_{\gtag^\prime_i}$ is $\oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_1)$ instead of $\oneSDFE.\Enc(\pk_{\gtag^\prime_i},x_\coin)$.
% In $\hybij{3}{i}$ and $\hybij{4}{i}$, we do not need randomness to generate $\pk_{\gtag^\prime_i}$ and $\ct_{\gtag^\prime_i}$.
% We just hardwire $\pk_{\gtag^\prime_i}$ and $\ct_{\gtag^\prime_i}$ into $\sfS^*_\sfonefe$ and $\sfE^*_\sfonefe$, respectively.
% In addition, it holds that $f_k(x_0)=f_k(x_1)$ for all $k\in[q]$ by the requirement of strong $\gamma$-anti-piracy security. For every $i \in [q]$, by the adaptive security of $\oneSDFE$ under the public key $\pk_{\gtag^\prime_i}$, $D^{(4,i)}$ is computationally indistinguishable from $D^{(3,i)}$.
% The detail of this indistinguishability is almost the same as~\cref{lem:ind-by-one-pkfe} and we omit it.

% In this hybrid game, we also use $\ATI^{\epsilon,\delta}_{\cE_b,D^{(4,i)},\frac{1}{2}+\gamma-\epsilon- (24i-9) \epsilon}$ instead of $\ATI^{\epsilon,\delta}_{\cE_b,D^{(3,i)},\frac{1}{2}+\gamma-(24i-12)\epsilon}$.

% By~\cref{cor:ind_distribution_ATI}, it holds that
% \begin{align}
% & \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(4,i)},\frac{1}{2}+\gamma -\epsilon -(24i-9)\epsilon}\tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(4,i)},\frac{1}{2} +\gamma -\epsilon -(24i-9)\epsilon})\qstateq] \\
% & \ge \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(3,i)},\frac{1}{2}+\gamma-\epsilon -(24i-12)\epsilon} \tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(3,i)},\frac{1}{2} +\gamma -\epsilon -(24i-12)\epsilon})\qstateq] - 3\delta.
% \end{align}
% That is, it holds that $\Adv_{4}^{i} \ge  \Adv_{3}^{i} - \negl(\secp)$.

% \item[$\hybij{5}{i}$:] This is defined for $i\in [q]$ and the same as $\hybij{4}{i}$ except that we use distribution $D^{(5,i)}$, which is the same as $D^{(4,i)}$ except that we use $r_{i} = \prf_{\prfkey}(\gtag^\prime_i)$ and $r^\prime_{i} = \prf^\prime_{\prfkey^\prime}(\gtag^\prime_i)$.
% By the punctured pseudorandomness of $\prf$ and $\prf^\prime$, $D^{(5,i)}$ is computationally indistinguishable from $D^{(4,i)}$.

% In this hybrid game, we also use $\ATI^{\epsilon,\delta}_{\cE_b,D^{(5,i)},\frac{1}{2}+\gamma-\epsilon- (24i-3) \epsilon}$ instead of $\ATI^{\epsilon,\delta}_{\cE_b,D^{(4,i)},\frac{1}{2}+\gamma-(24i-9)\epsilon}$.

% By~\cref{cor:ind_distribution_ATI}, it holds that
% \begin{align}
% & \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(5,i)},\frac{1}{2}+\gamma -\epsilon -(24i-3)\epsilon}\tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(5,i)},\frac{1}{2} +\gamma -\epsilon -(24i-3)\epsilon})\qstateq]  \\
% & \ge \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(4,i)},\frac{1}{2}+\gamma -\epsilon -(24i-9)\epsilon} \tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(4,i)},\frac{1}{2} +\gamma -\epsilon -(24i-9)\epsilon})\qstateq] - 3\delta.
% \end{align}

% We finish describing one cycle of our hybrid games.
% We move from $\hybij{5}{i}$ to $\hybij{1}{i+1}$.
% From the definition of $\sfS^*_{\sfonefe}$ and $\hybij{1}{i}$, the behaviors of $\sfS^*_{\sfonefe}$ in $\hybij{5}{i}$ and $\hybij{1}{i+1}$ are the same.
% By~\cref{cor:ind_distribution_ATI} and the indistinguishability of $\iO_1$, it holds that
% \begin{align}
% & \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(1,i+1)},\frac{1}{2}+\gamma -\epsilon -(24i)\epsilon}\tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(1,i+1)},\frac{1}{2} +\gamma -\epsilon -(24i)\epsilon})\qstateq]  \\
% &\ge \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(5,i)},\frac{1}{2}+\gamma -\epsilon -(24i-3)\epsilon} \tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(5,i)},\frac{1}{2} +\gamma -\epsilon -(24i-3)\epsilon})\qstateq] - 3\delta.
% \end{align}
% That is, $\Adv_{1}^{i+1} \ge  \Adv_{5}^{i}  - \negl(\secp)$ holds.

% \item[$\hybij{4}{q+1}$:] This is the same as $\hybij{3}{q+1}$ except that we change the distribution $D^{(3,q+1)}$ over pairs $(\coin,\ct)$ into $D^{(4,q+1)}$ as follows.
% \begin{itemize}
%  \item Sample a uniform $\coin \chosen \bit$.
%  \item Sample $r^\prime_{\gtag^\ast} \chosen \cR_{\Enc}$ and compute $\ct_{\gtag^\ast} \la \oneSDFE.\Enc(\pk_{\gtag^\ast},x_\coin ;r^\prime_{\gtag^\ast})$, $\prfkey^\prime \la \prfgen^\prime(1^\secp)$, $\prf^\prime_{\ne \gtag^\ast} \la \Puncture^\prime(\prfkey^\prime,\gtag^\ast)$, and $\cthat \gets \iO_2(\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}])$ where $\sfE^{\ast\ast}_\sfonefe$ is described in~\cref{fig:enc-one-sdfe-punc-last}. Set $\ct \seteq \cthat$.
%  \end{itemize} 


% \protocol
% {Encryption Circuit $\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast}, x_1,\ct_{\gtag^\ast}](\gtag)$}
% {Circuit $\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}]$.
% }
% {fig:enc-one-sdfe-punc-last}
% {
% \ifnum\llncs=1
% \scriptsize
% \else
% \fi
% \begin{description}
% \setlength{\parskip}{0.3mm} % between paragraph
% \setlength{\itemsep}{0.3mm} % between items
% \item[Hardwired:] tag $\gtag^\ast$, public key $\pkhat$ (this is an obfuscated circuit), puncturable PRF key $\prf^\prime_{\ne \gtag^\ast}$, plaintext $x_1$, and ciphertext $\ct_{\gtag^\ast}$.
% \item[Input:] tag $\gtag \in \zo{\ell}$.
% \item[Padding:] circuit is padded to size $\padsize_{\sfE}\seteq\padsize_{\sfE}(\secp,n,s)$, which is determined in analysis.
% \end{description}
% \begin{enumerate}
% \setlength{\parskip}{0.3mm} % between paragraph
% \setlength{\itemsep}{0.3mm} % between items
% \item If $\gtag^\ast = \gtag$, output $\ct_{\gtag^\ast}$.
% \item Else, compute $r^\prime_{\gtag} \gets \prf^\prime_{\ne \gtag^\ast}(\gtag)$ and the circuit $\pkhat$ on input $\gtag$, that is, $\pk_{\gtag} \gets \pkhat(\gtag)$,
% \item Output $\ct_{\gtag} \gets \oneSDFE.\Enc(\pk_{\gtag},x_1;r^\prime_{\gtag})$.
% \end{enumerate}
% }

% From the definitions of $\sfE^\ast_{\sfonefe}$, $\sfE^{\ast\ast}_{\sfonefe}$, and $\hybij{3}{q+1}$, the behaviors of $\sfE^{\ast}_{\sfonefe}$ in $\hybij{3}{q+1}$ is the same as that of $\sfE^{\ast\ast}_{\sfonefe}$ in $\hybij{4}{q+1}$.
% Moreover, both circuits have the same size by padding $\pad_\sfE$. Then, we can use the indistinguishability guarantee of $\iO_2$ and it holds that $D^{(4,q+1)}$ is computationally indistinguishable from $D^{(3,q+1)}$.
% This change is for erasing information about $\coin$ from $\sfE^{\ast}_{\sfonefe}$.

% By~\cref{cor:ind_distribution_ATI}, it holds that
% \begin{align}
% & \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(4,q+1)},\frac{1}{2}+\gamma -\epsilon -(24q+15)\epsilon}\tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(4,q+1)},\frac{1}{2} +\gamma  -\epsilon -(24q+15)\epsilon})\qstateq]  \\
% &\ge \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(3,q+1)},\frac{1}{2}+\gamma -\epsilon-(24q+12)\epsilon} \tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(3,q+1)},\frac{1}{2} +\gamma -\epsilon -(24q+ 12)\epsilon})\qstateq] - 3\delta.
% \end{align}
% That is, it holds that $\Adv_{4}^{q+1} \ge  \Adv_{3}^{q+1} - \negl(\secp)$.

% \item[$\hybi{6}$:] This is the same as $\hybij{4}{q+1}$ except that we generate a PRF key $\prfkey_1 \gets \prfgen_1(1^\secp)$ and $\prfkey_2 \gets \prfgen_2(1
% ^\secp)$ at the beginning of the game and change the distribution $D^{(4,q+1)}$ over pairs $(\coin,\ct)$ into $D^{(6)}$ as follows.
% \begin{itemize}
%  \item Sample a uniform $\coin \chosen \bit$.
%  \item Sample $r^\prime_{\gtag^\ast} \chosen \cR_{\Enc}$, compute $\ct_{\gtag^\ast} \la \oneSDFE.\Enc(\pk_{\gtag^\ast},x_\coin ;r^\prime_{\gtag^\ast})$, $r_1\gets \prf_1(\prfkey_1,\ct_{\gtag^\ast})$, $r_2\gets \prf_2(\prfkey_2,\ct_{\gtag^\ast})$, $\prfkey^\prime \la \PRF^\prime.\Gen(1^\secp;r_1)$, $\prf^\prime_{\ne \gtag^\ast} \la \Puncture^\prime(\prfkey^\prime,\gtag^\ast)$, and $\cthat \gets \iO_2(\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}];r_2)$ where $\sfE^{\ast\ast}_\sfonefe$ is described in~\cref{fig:enc-one-sdfe-punc-last}. Set $\ct \seteq \cthat$.
%  \end{itemize} 
%  That is, we de-randomize generation of $\prfkey^\prime$ and $\cthat$. Note that the puncturing algorithm $\Puncture^\prime$ is deterministic in the GGM construction~\cite{JACM:GolGolMic86,AC:BonWat13,CCS:KPTZ13,PKC:BoyGolIva14}.
% By the pseudorandomness of $\PRF_1$ and $\PRF_2$, $D^{(6)}$ is computationally indistinguishable from $D^{(4,q+1)}$.

% By~\cref{cor:ind_distribution_ATI}, it holds that
% \begin{align}
% & \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(6)},\frac{1}{2}+\gamma -\epsilon -(24q+21)\epsilon}\tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(6)},\frac{1}{2} +\gamma  -\epsilon -(24q+21)\epsilon})\qstateq]  \\
% &\ge \Tr[(\ATI^{\epsilon,\delta}_{\cE_1,D^{(4,q+1)},\frac{1}{2}+\gamma -\epsilon-(24q+15)\epsilon} \tensor \ATI^{\epsilon,\delta}_{\cE_2,D^{(4,q+1)},\frac{1}{2} +\gamma -\epsilon -(24q+ 15)\epsilon})\qstateq] - 3\delta.
% \end{align}
% That is, it holds that $\Adv_{6} \ge  \Adv_{4}^{q+1} - \negl(\secp)$.
% Note that we use~\cref{cor:ind_distribution_ATI} two times here since we use both $\PRF_1$ and $\PRF_2$.
% \fuyuki{I do not see why we need to use ~\cref{cor:ind_distribution_ATI} twice although $D^{(4,q+1)}$ and $D^{(6)}$ are computationally indistinguishable distributions.}
% \end{description}

% We prove the following.
% \begin{lemma}\label{lem:1SDFE_reduction}
% If $\oneSDFE$ is challenge-only strong $\gamma/2$-anti-piracy secure, it holds that $\Adv_{6} \le \negl(\secp)$.
% \end{lemma}
% \begin{proof}[Proof of~\cref{lem:1SDFE_hyb1}]
% Suppose that $\Adv_{4}^{q+1}$ is non-negligible for a contradiction.
% We construct a QPT algorithm $\qB$ for the strong $\gamma/2$-anti-piracy game of $\oneSDFE$ by using the adversary $\qA$ of the strong $\gamma$-anti-piracy game of $\SDFE$ as follows.
% \begin{enumerate}
% \item  $\qB$ chooses $\gtag_1,\ldots,\gtag_q \chosen \zo{\ell}$ and generates $\prfkey \gets \prfgen(1^\secp)$, $\prfkey_1 \gets \prfgen_1(1^\secp)$, and $\prfkey_2 \gets \prfgen_2(1^\secp)$.
% \item $\qB$ generates $\prf_{\ne \gtag^\ast} \la \Puncture(\prfkey,\gtag^\ast)$. % and $\prfkey^\prime_{\ne \gtag^\ast} \la \Puncture^\prime(\prfkey^\prime,\gtag^\ast)$.
% \item $\qB$ receives $\pk^\ast$ from its challenger, sets $\pk_{\gtag^\ast} \seteq \pk^\ast$, and constructs $\sfS^*_\sfonefe[\gtag^\ast,\prf_{\ne \gtag^\ast},\pk_{\gtag^\ast}]$ described in~\cref{fig:setup-sdfe-punc} by choosing $\gtag^\ast$ for the challenge query $f^\ast$.
% $\qB$ sets $\pkhat \seteq \iO_1(\sfS^*_\sfonefe[\gtag^\ast,\prf_{\ne \gtag^\ast},\pk_{\gtag^\ast}])$ and sends it to $\qA$.
% \item When $\qA$ sends a key query $f_i$, $\qB$ generates $(\pk_{\gtag_i},\msk_{\gtag_i})\gets \oneSDFE.\Setup(1^\secp;\PRF_{\prfkey_{\ne \gtag^\ast}}(\gtag_i))$ and $\qsk_{f_i,\gtag_i} \gets \oneSDFE.\QKeyGen(\msk_{\gtag_i},f_i)$, sets $\qskhat_{f_i,\gtag_i} \seteq (\gtag_i,\qsk_{f_i,\gtag_i})$, and sends $\qskhat_{f_i}$ to $\qA$.
% \item When $\qA$ sends the challenge query $f^\ast$, $\qB$ passes it to its challenger and receives $\qsk_{f^\ast} \gets \oneSDFE.\QKeyGen(\msk^\ast,f^\ast)$, and sends $\qskhat_{f^\ast} \seteq (\gtag^\ast,\qsk_{f^\ast})$ to $\qA$.
% \item Again, $\qB$ can answer key queries $f_i$ from $\qA$ as the fourth item.
% \item At some point, $\qB$ receives $(x_0,x_1)$ and two (possibly entangled) quantum decryptors $\pirateD_1 = (\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2 = (\qstateq[\qreg{R}_2],\mat{U}_2)$, where $f^*(x_0)\ne f^*(x_1)$, from $\qA$. For $i\in \setbk{1,2}$, let $\cP_{i,D^{(4,q+1)}}$ be the following mixture of projective measurements acting on some quantum state $\qstateq^\prime$:
% \begin{itemize}
%  \item Sample a uniform $\coin \chosen \bit$.
%  \item Sample $r^\prime_{\gtag^\ast} \chosen \cR_{\Enc}$, $\ct_{\gtag^\ast} \la \oneSDFE.\Enc(\pk_{\gtag^\ast},x_\coin ;r^\prime_{\gtag^\ast})$.
% \item Generate $r_1\gets \prf_1(\prfkey_1,\ct_{\gtag^\ast})$, $r_2\gets \prf_2(\prfkey_2,\ct_{\gtag^\ast})$, $\prfkey^\prime \gets \prfgen^\prime(1^\secp;r_1)$, and $\prf^\prime_{\ne \gtag^\ast}=\Puncture^\prime(\prfkey^\prime,\gtag^\ast)$.
% \item Generate $\cthat \gets \iO_2(\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}];r_2)$ where $\sfE^{\ast\ast}_\sfonefe$ is described in~\cref{fig:enc-one-sdfe-punc-last}.
%  \item Run the quantum decryptor $(\qstateq^\prime,\mat{U}_i)$ on input $\cthat$. If the outcome is % $f^\ast(x_\coin)$,
%  $\coin$, output $1$. Otherwise, output $0$.
% \end{itemize}
% $\qB$ runs $\ATI^{\epsilon,\delta}_{\cE_1,D^{(4,q+1)},\frac{1}{2}+\gamma -\epsilon -(24q+21)\epsilon}$ and $\ATI^{\epsilon,\delta}_{\cE_2,D^{(4,q+1)},\frac{1}{2}+\gamma -\epsilon -(24q+21)\epsilon}$ on quantum decryptor $\pirateD_1=(\qstateq[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2=(\qstateq[\qreg{R}_2],\mat{U}_2)$.
% $\qB$ aborts if either of the tests does not pass, otherwise proceeds to the next step.
% Let $\qstateq^\ast$ be the bipartite state conditioned on both outcomes being $1$.
% \item $\qB$ sets quantum decryptors $\pirateD_1^\ast$ and $\pirateD_2^\ast$ as follows.

% In this item, we denote pure state $\ket{x}\bra{x}$ by $\ket{x}$ for ease of notation.
% First, $\qB$ constructs $(\qstateq^\ast[\qreg{R}_i],\mat{U}_i^\ast)$ such that
% \begin{itemize}
% \item Set  $\qstateq^\ast[\qreg{R}_i] \seteq \qstateq[\qreg{R}_i] \tensor \ket{0^{\abs{\cthat}}} \tensor \ket{\gtag^\ast, \pkhat, 0^\ell, x_1, \prfkey_1,\prfkey_2,0^{\abs{r_1}},0^{\abs{r_2}},0^{\ell}} \tensor \ket{\ct_{\gtag^\ast}}$. Note that $\ket{\ct_{\gtag^\ast}}$ is the input for $\qstateq^\ast[\qreg{R}_i]$.
% \item Unitary $\mat{U}^\ast_i$ acts on $\qstateq^\ast[\qreg{R}_i]$ and the result is
% \[
% \qstateq^\prime[\qreg{R}_i] \seteq \qstateq[\qreg{R}_i] \tensor \ket{\cthat} \tensor \ket{\gtag^\ast, \pkhat, \prf^\prime_{\ne \gtag^\ast}, x_1,\prfkey_1,\prfkey_2,r_1,r_2,\prfkey^\prime}\tensor \ket{\ct_{\gtag^\ast}},
% \]
% where $r_1 \seteq \prf_1(\prfkey_1,\ct_{\gtag^\ast})$, $r_2 \seteq \prf_2(\prfkey_2,\ct_{\gtag^\ast})$, $\prfkey^\prime \seteq \prfgen^\prime(1^\secp;r_1)$, $\prf^\prime_{\ne \gtag^\ast} \seteq \Puncture^\prime(\prfkey^\prime,\gtag^\ast)$, $\cthat \seteq  \iO_2(\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}];r_2)$. That is, $\mat{U}_i$ constructs $\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}]$ described in~\cref{fig:enc-one-sdfe-punc-last} and generates $\cthat \seteq \iO_2(\sfE^{\ast\ast}_\sfonefe[\gtag^\ast,\pkhat,\prf^\prime_{\ne \gtag^\ast},x_1,\ct_{\gtag^\ast}];r_2)$. Note that $\qB$ can construct it since $\qB$ has $\gtag^\ast$, $\pkhat$, $\prfkey_1$, $\prfkey_2$, and $x_1$.
% \end{itemize}
% It is easy to see that if we apply $(\mat{U}_i \tensor \mat{I})$ to $\qstateq^\prime[\qreg{R}_i]$, we obtain an output of $\pirateD_i$ for input $\cthat$.
% Thus, $\qB$ sets $\pirateD_1^\ast \seteq (\qstateq^\ast[\qreg{R}_1],(\mat{U}_1\tensor \mat{I})\mat{U}_1^\ast)$ and $\pirateD_2^\ast \seteq (\qstateq^\ast[\qreg{R}_2],(\mat{U}_2 \tensor \mat{I})\mat{U}_2^\ast)$.
% $\qB$ sends $(x_0,x_1)$ and $\pirateD_1^\ast$ and $\pirateD_2^\ast$ to its challenger.
% \end{enumerate}
% By the construction of $\mat{U}_i^\ast$, quantum decryptor $\pirateD_i^\ast$ takes a ciphertext $\ct_{\gtag^\ast}$ under $\pk_{\gtag^\ast}$ as input, converts it into a ciphertext $\cthat$ of $\SDFE$, and apply the quantum decryptor $\pirateD_i$ from $\qA$. The converted ciphertext $\cthat$ perfectly simulates a ciphertext in $\hybi{6}$ if an input to $\pirateD_i^\ast$ is a ciphertext under $\pk_{\gtag^\ast}$.


% We assumed that $\Adv_{6}$ is non-negligible at the begging of this proof.
% That is, applying $\ATI^{\epsilon,\delta}_{\cE_i,D^{(4,q+1)},\frac{1}{2}+\gamma -\epsilon -(24q+21)\epsilon}$ on $\qstateq^\ast[\qreg{R}_i]$ results in two outcomes $1$ with non-negligible probability.
% By the second item of~\cref{lem:ATI_bipartite_app}, it holds that
% \begin{align}
% \Tr[\TI_{\frac{1}{2}+\gamma -(24q+21)\epsilon- 3\epsilon}(\cP_{1,D^{(6)}}) \tensor \TI_{\frac{1}{2}+\gamma - (24q+21)\epsilon- 3\epsilon}(\cP_{2,D^{(6)}})\qstateq^\ast] \ge 1- 4\delta.
% \end{align}
% This means that for $i\in \setbk{1,2}$, $\qstateq^\ast[\qreg{R}_i]$ is negligibly close to being a $(\gamma -(24q+21)\epsilon-3\epsilon)$-good decryptor with respect to ciphertexts generated according to $D^{(6)}$.


% Thus, if $\pirateD_i$ works as a $\gamma$-good quantum decryptor for $\SDFE$, $\pirateD_i^\ast$ works as a $(\gamma - (24q+21) \epsilon - 3\epsilon)$-good quantum decryptor for $\oneSDFE$, where $\epsilon= \frac{\gamma}{2(24q+24)}$. This completes the proof of~\cref{lem:1SDFE_reduction}.
% \end{proof}

% By using the relationships among $\adva{\SDFE,\qA}{}$, $\Adv_{1}^{0}$, $\Adv_{x}^{i}$ for $x\in \setbk{1,\cdots,5}$ and $i\in [q]$, $\Adv_{x}^{q+1}$ for $x\in \setbk{1,\cdots,4}$, and $\Adv_6$ that we show above, we obtain $\advc{\SDFE,\qA}{strong}{anti}{piracy}(\secp,\gamma) \le \negl(\secp)$.
% \end{proof}
